Weighted Scheduling of Time-Sensitive Coflows

Datacenter networks commonly facilitate the transmission of data in distributed computing frameworks through coflows, which are collections of parallel flows associated with a common task. Most of the existing research has concentrated on scheduling coflows to minimize the time required for their completion, i.e., to optimize the average dispatch rate of coflows in the network fabric. Nevertheless, modern applications often produce coflows that are specifically intended for online services and mission-crucial computational tasks, necessitating adherence to specific deadlines for their completion. In this paper, we introduce \wdcoflow,~ a new algorithm to maximize the weighted number of coflows that complete before their deadline. By combining a dynamic programming algorithm along with parallel inequalities, our heuristic solution performs at once coflow admission control and coflow prioritization, imposing a $\sigma$-order on the set of coflows. With extensive simulation, we demonstrate the effectiveness of our algorithm in improving up to $3\times$ more coflows that meet their deadline in comparison the best SoA solution, namely $\mathtt{CS\text{-}MHA}$. Furthermore, when weights are used to differentiate coflow classes, \wdcoflow~ is able to improve the admission per class up to $4\times$, while increasing the average weighted coflow admission rate.

==> sections/Heuristics-oldversion.tex <==
%!TEX root=main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposed Heuristic Algorithm 
\section{$\sigma$-Order Scheduling with $\mathtt{DCoflow}$ 
\label{sec:heuristic}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we present $\mathtt{DCoflow}$, an algorithm to solve the problem of joint coflow admission control and scheduling. Given a list of $N$ coflows, it provides a permutation $\sigma=(\sigma_1,\sigma_2,..,\sigma_N)$ of these coflows, with the aim of maximizing the coflow acceptance rate. We observe that, when a coflow is served according to the corresponding $\sigma$-order-preserving schedule, lower-priority coflows will be impacted. It is hence possible that some of these lower-priority coflows will not respect their deadline. Hence our objective is to evaluate the impact of a scheduled coflow with respect to the original CAR problem. The problem is combinatorial in nature, since there are $N!$ possible coflow orderings. Hence, we propose a new approach that uses the formulation of Problem~\eqref{prob:ILP}  by deriving a necessary condition  satisfied by all feasible coflow orders solving Problem~\eqref{prob:ILP}. 

Consider a feasible solution to Problem~\eqref{prob:ILP} and  a subset $\cS \subseteq \cC$ of coflows. Given a coflow $k \in \cC$, let $\cS_k^-=\left \{ k' \in \cS \ : \ \delta_{k',k} = 1\right \}$ be the set of coflows in $\cS$ which are scheduled before $k$. Condition \eqref{eq:lower-bound-CCT} may be rewritten as
\begin{equation}
c_{\ell,k} \geq p_{\ell,k} + \sum_{k' \in \cS_k^-} p_{\ell,k'} z_{k'},
\label{eq:parallel-inequalities-1}
\end{equation}
which implies
\begin{equation}
c_{\ell,k} p_{\ell,k} z_k \geq p_{\ell,k}^2 z_k^2 + p_{\ell,k} z_k \sum_{k' \in \cS_k^-} p_{\ell,k'} z_{k'}.
\label{eq:parallel-inequalities-2}
\end{equation}

Using the inequality $T_k \geq c_{\ell,k} z_k $ and summing over all coflows $k \in \cS$, we obtain
% \begin{eqnarray}
% \sum_{k \in \cS} p_{\ell,k} T_k & \geq & \sum_{k \in \cS} c_{\ell,k} p_{\ell,k} z_k, \nonumber \\
% & \geq & \sum_{k \in \cS} \left ( p_{\ell,k} z_k \right )^2 +  \sum_{k \in \cS}  p_{\ell,k} z_k \sum_{k' \in \cS_k^-} p_{\ell,k'} z_{k'} \nonumber \\
% & = & \frac{1}{2} \sum_{k \in \cS} \left ( p_{\ell,k} z_k \right )^2 +  \nonumber \\
% &   & \frac{1}{2} \left [ \sum_{k \in \cS} \left ( p_{\ell,k} z_k \right )^2 + 2 \sum_{k \in \cS}  p_{\ell,k} z_k \sum_{k' \in \cS_k^-} p_{\ell,k'} z_{k'} \right ]  \nonumber \\
% & = & \frac{1}{2}  \sum_{k \in \cS} \left ( p_{\ell,k} z_k \right )^2 +  \frac{1}{2}  \left ( \sum_{k \in \cS}  p_{\ell,k} z_k \right )^2.  \label{eq:parallel-inequalities-3} 
% \end{eqnarray}
% \begin{align}
% \sum_{k\in\mathcal{S}}p_{\ell,k}T_{k}\geq & \sum_{k\in\mathcal{S}}c_{\ell,k}p_{\ell,k}z_{k},\nonumber \\
% \geq & \sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+\sum_{k\in\mathcal{S}}p_{\ell,k}z_{k}\sum_{k'\in\mathcal{S}_{k}^{-}}p_{\ell,k'}z_{k'}\nonumber \\
% = & \frac{1}{2}\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+\nonumber \\
%  & \frac{1}{2}\left[\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+2\sum_{k\in\mathcal{S}}p_{\ell,k}z_{k}\sum_{k'\in\mathcal{S}_{k}^{-}}p_{\ell,k'}z_{k'}\right]\nonumber \\
% = & \frac{1}{2}\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+\frac{1}{2}\left(\sum_{k\in\mathcal{S}}p_{\ell,k}z_{k}\right)^{2}.\label{eq:parallel-inequalities}
% \end{align}
\begin{small}
\begin{align} 
\sum_{k\in\mathcal{S}}p_{\ell,k}T_{k} \geq & \sum_{k\in\mathcal{S}}c_{\ell,k}p_{\ell,k}z_{k} \geq   \sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2} + \hskip-4mm \sum_{k\in\mathcal{S}, k'\in\mathcal{S}_{k}^{-}} \hskip-4mm
p_{\ell,k}p_{\ell,k'}z_{k}z_{k'}\nonumber \\
 & \hskip-19mm=\frac{1}{2}\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+\nonumber \frac{1}{2}\left[\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+2\sum_{k\in\mathcal{S}}p_{\ell,k}z_{k} \hskip-2mm \sum_{k'\in\mathcal{S}_{k}^{-}}p_{\ell,k'}z_{k'}\!\right]\nonumber \\
&\hskip-19mm = \frac{1}{2}\sum_{k\in\mathcal{S}}\left(p_{\ell,k}z_{k}\right)^{2}+\frac{1}{2}\left(\sum_{k\in\mathcal{S}}p_{\ell,k}z_{k}\right)^{2}.\label{eq:parallel-inequalities}
\end{align}
\end{small}
We thus conclude that any feasible solution to Problem~\eqref{prob:ILP} satisfies the condition $\sum_{k \in \cS} p_{\ell,k} T_k \geq f_\ell(\cS)$ for any subset $\cS \subseteq \cC$ of \emph{accepted} coflows, where $f_\ell(\cS)=\frac{1}{2}  \sum_{k \in \cS} p_{\ell,k}^2 +  \frac{1}{2}  \left ( \sum_{k \in \cS}  p_{\ell,k} \right )^2$. These conditions are the so-called \textit{parallel inequalities} and provide valid inequalities for the concurrent open shop problem \cite{Mastrolilli2010}. Note that they do not depend on the ordering of the coflows. 

We shall use the parallel inequalities to determine the coflows that should not be admitted. Consider a solution to Problem~\eqref{prob:ILP} and assume that, in this solution, there exists a subset $\cS$ of accepted coflows (i.e., $z_k=1$ 
for all $k \in \cS$) such that $\sum_{k \in \cS} p_{\ell,k} T_k < f_\ell(\cS)$ for at least one port $\ell \in \cL$. This implies that this solution is not feasible and can only become feasible by rejecting a coflow $k'$ among the accepted coflows using port $\ell$. We choose this coflow $k'$ so as to minimize the quantity $f_\ell(\cS \setminus \{ k' \}) - \sum_{k \in \cS \setminus \{ k' \}} p_{\ell,k} T_k$, in the hope that it becomes negative. Observe that 

\vspace{-0.5cm}
\begin{small}
\begin{align}
f_{\ell}\left(\cS \right) & \! =\!   \left [ \frac{1}{2}p_{\ell,k'}^{2}\! +\! \frac{1}{2}\! \sum_{k \in \cS \setminus \{ k' \} } p_{\ell,k}^{2} \right ] \! +\!  \frac{1}{2}\!  \left ( p_{\ell k'}+\! \sum_{k \in \cS \setminus \{ k' \} }p_{\ell k} \right )^{2} \nonumber \\
 & =  f_{\ell} \left ( \cS \setminus \{ k' \} \right ) + p_{\ell, k'} \sum_{k \in \cS} p_{\ell,k}, \label{eq:fls_split}
\end{align}
\end{small}
from which it follows that
\begin{small}
\begin{align}
f_{\ell}\left(\cS \setminus \{ k' \} \right)- \sum_{k \in \cS \setminus \{ k' \} } p_{\ell,k}T_k  & =
f_{\ell} \left(\cS \right) - \sum_{k \in \cS} p_{\ell,k} T_k  \nonumber \\
 &  + p_{\ell, k'} \left ( T_{k'}-\sum_{k \in\cS} p_{\ell,k} \right )\label{eq:fls_constraint_split}
\end{align}
\end{small}
The above relation will be used to define our coflow admission control algorithm. In general, it suggests possible heuristics to remove a coflow $k'$ from $\cS$ in order to satisfy the parallel inequalities. For instance, one such heuristics is to minimize the quantity 
\begin{equation}
\Psi_{\ell,k'} := p_{\ell,k'} \left ( T_{k'}-\sum_{k \in \cS} p_{\ell,k} \right ).  
\end{equation}
In fact, the term $\sum_{k \in \cS} p_{\ell,k} - T_{k'}$ represents how much the completion time of coflow $k'$ on port $\ell$ exceeds its deadline, assuming that it is scheduled latest. Hence, we could reject coflow $k'$ with both large processing time $p_{\ell,k'}$ on port $\ell$ and large deadline violation. More admission rationales based on \eqref{eq:fls_constraint_split} will be detailed in  describing $\mathtt{DCoflow}$, whose pseudocode is reported in Algorithm~\ref{algo:DCoflow}. Generally, $\mathtt{DCoflow}$ takes a list of unsorted coflows and provides as output the scheduling order of accepted coflows. It works in rounds and at each round, it either accepts a coflow or it rejects one. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PARTIE COMMENTEE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{comment}
% It can be seen that the constraint \eqref{eq:AdaptOptim:Quad} has
% a quadratic form, thus makes $\mathtt{MaxCdsReduced}$ harder to solve.
% In what follows, we introduces a heuristic based on the constraint
% \eqref{eq:AdaptOptim:Quad} of $\mathtt{MaxCdsReduced}$. 

% Denote $f_{\ell}\left(\mathcal{S}\right)=\frac{1}{2}\sum_{j\in\mathcal{S}}p_{\ell j}^{2}+\frac{1}{2}\left(\sum_{j\in\mathcal{S}}p_{\ell j}\right)^{2}$
% and consider $x$ is the last scheduled coflow in $\mathcal{S}$,
% one has\vspace{-0.5cm}


% From \eqref{eq:fls_constraint_deadline} and \eqref{eq:fls_split},
% one has
% \begin{scriptsize}
% \begin{align}
%  & f_{\ell}\left(\mathcal{S}\right)-\sum_{j\in\mathcal{S}}p_{\ell j}T_{j}\leq0\nonumber \\
%  & \Leftrightarrow f_{\ell}\left(\mathcal{S}\backslash\left\{ x\right\} \right)+p_{\ell x}\sum_{j\in\mathcal{S}}p_{\ell j}-\sum_{j\in\mathcal{S}}p_{\ell j}T_{j}\leq0\nonumber \\
%  & \Leftrightarrow f_{\ell}\left(\mathcal{S}\backslash\left\{ x\right\} \right)+p_{\ell x}\sum_{j\in\mathcal{S}}p_{\ell j}-\Big(p_{\ell x}T_{x}+\sum_{j\in\mathcal{S}\backslash\left\{ x\right\} }p_{\ell j}T_{j}\Big)\leq0\nonumber \\
%  & \Leftrightarrow\Big[f_{\ell}\left(\mathcal{S}\backslash\left\{ x\right\} \right)-\sum_{j\in\mathcal{S}\backslash\left\{ x\right\} }p_{\ell j}T_{j}\Big]-p_{\ell x}\Big(T_{x}-\sum_{j\in\mathcal{S}}p_{\ell j}\Big)\leq0.\label{eq:fls_constraint_split}
% \end{align}
% \end{scriptsize}
% It is observed that the first term in \eqref{eq:fls_constraint_split}
% is independent of $x$. So the criterion to select coflow $x\in\mathcal{S}$
% to be scheduled at the latest depends on the second term, $\Psi_{\ell x}=p_{\ell x}\Big(T_{x}-\sum_{j\in\mathcal{S}}p_{\ell j}\Big)$.
% Suppose that $x$ is the coflow that violates the deadline requirement,
% as we try to minimize the left-hand of \eqref{eq:fls_constraint_split}
% as much as possible, the coflow to be last scheduled should be the
% one that minimize $\Psi_{\ell x}$. Having this, we introduce the
% following algorithm.

% \end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FIN PARTIE COMMENTEE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $\mathtt{DCoflow}$ employs a two-step algorithm. First, it applies Algorithm~\ref{algo:DCoflow} to obtain the initial scheduling order $\sigma$ which contains all coflows in $\cC$. Then, $\mathtt{DCoflow}$ applies Algorithm~\ref{algo:RemoveLateCoflows} to estimate the CCT of all coflows and remove from $\sigma$ the coflows that do not satisfy the deadline constraint.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DCoflow ALGORITHM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\footnotesize
\caption{$\mathtt{DCoflow}$ \label{algo:DCoflow}}

\BlankLine

$\cS=\left \{ 1,2,\ldots, N \right \}$; \Comment{initial set of unscheduled
coflows}

$\sigma = \varnothing;$ \Comment{initial scheduling order}

$\sigma^{\star} = \varnothing;$ \Comment{initial set of pre-rejected coflows}

$n = N$;  \Comment{round counter}

\While{ $\cS \neq \varnothing$ }{

	%$\ell_b = \underset{\ell \in {\cL}}{\mathrm{arg\,max}}\, \left \{  { r_{\ell} + \sum_{k \in \cS}}p_{\ell, k} \right \}$; \Comment{bottleneck port}
    
    $\ell_b = \underset{\ell \in {\cL}}{\mathrm{arg\,max}}\,  \sum_{k \in \cS} p_{\ell, k}$; \Comment{bottleneck port}
    
	% {\it \# Determine the set of coflows using $\ell_b$}

	$\cS_{\ell_b} = \left\{ k \in {\cS} : p_{\ell_b, k} > 0 \right\}$; \Comment{set of coflows using $\ell_b$}

	{\it \# Coflows that can finish in time when scheduled last}

	$\cS^d_{\ell_b}\leftarrow \{j\in \cS_{\ell_b} |  \sum_{k \in \cS_{\ell_b}} p_{\ell_b,k} \leq T_j\}$; 

	\eIf{$\displaystyle \cS^d_{\ell_b} \not = \varnothing$}
	{
		%{\it \# Select coflow with largest deadline to admit}
		
		%$k_n = \mathtt{AdmittedCoflow} \Big(\cS^d_{\ell_b},(T_k)_{k\in\cS^d_{\ell_b}} \Big)$; 
        $k_n = \underset{k \in {\cC}}{\mathrm{arg\,max}} \, T_k $; \Comment{admit coflow with largest deadline}
        
		% Choose $i \in \underset{x \in *\cS_{\ell_b}}{\mathrm{arg\,max}}\,  T_x$;
		 
		$\sigma_{n} = k_n$; \Comment{append $k_n$ to $\sigma$} 

		$\cS = \cS \setminus \left\{ k_n \right\} $; \Comment{remove $k_n$ from $\cS$} 

	}{
		%{\it \# Select a coflow to reject}
		
		$k^{\star} = \mathtt{RejectedCoflow}(\cS)$; \Comment{select a coflow to reject}
		
		$\sigma_{n} = k^{\star}$; \Comment{append $k^{\star}$ to $\sigma$}; 
		
		$\sigma^{\star} = \sigma^{\star} \cup \left\{ k^{\star} \right\}$; \Comment{append $k^{\star}$ to $\sigma^{\star}$}

		$\cS = \cS \backslash \left\{ k^{\star} \right\}$; \Comment{remove $k^{\star}$ from $\cS$} 

	} %EndIf
	
	$n = n-1$; \Comment{update the round index} 

} %EndWhile
$\sigma = \mathtt{RemoveLateCoflows} \left( \sigma, \sigma^{\star} \right)$; 

\KwRet $\sigma$;  \Comment{final scheduling order}

\vspace{0.1cm}

\SetKwFunction{FMain}{RemoveLateCoflows} 

\SetKwProg{Fn}{Function}{:}{} 

% \KwInput{Your Input}

\Fn{\FMain{\textit{$\sigma$, $\sigma^{\star}$}}}{ 

% \textit{\# Calculate the CCT of all coflows $\sigma_{k}$ in $\sigma$}

% $c_{\sigma_{k}}\leftarrow\mathtt{evalCCT}\left(\left\{ \sigma_{k}\right\} _{k\in[1,N]}\right)$,
% $\forall k\in[1,N]$;

% \textit{\# Determine the set of pre-rejected coflows $\sigma^{\star}$}

% $\sigma^{\star}=\left\{ \sigma_{k}\in\sigma:c_{\sigma_{k}}>T_{\sigma_{k}}\right\} $

\While{ $\sigma^{\star}\neq\varnothing$ }{

% \textit{\# Consider the first coflow in the set $\sigma^{\star}$}

$k^{\star}\leftarrow\underset{k}{\mathrm{arg\,min}}\left\{ \sigma_{k}\in\sigma^{\star}\right\} $; \Comment{first coflow in $\sigma^{\star}$}

% \textit{\# Calculate the CCT of coflow $\sigma_{k^{\star}}$}

$c_{\sigma_{k^{\star}}}\leftarrow\mathtt{evalCCT}\left(\left\{ \sigma_{k}\right\} _{k\in\left[1,k^{\star}\right]}\right)$; \Comment{CCT of coflow $\sigma_{k^{\star}}$}

\If{ $c_{\sigma_{k^{\star}}} > T_{\sigma_{k^{\star}}}$}{
$\sigma\leftarrow\sigma\backslash\left\{ \sigma_{k^{\star}}\right\} $;
} %EndIf
$\sigma^{\star}\leftarrow\sigma^{\star}\backslash\left\{ \sigma_{k^{\star}}\right\} $;
} %EndWhile
\KwRet $\sigma$;  
} %EndFunction
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END OF ALGORITHM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

$\mathtt{DCoflow}$ starts by computing the total completion time at each port and finds the bottleneck $\ell_b$, i.e., the port with the largest completion time. Having this, it determines $\mathcal{S}^d_{\ell_b}$, the set of coflows active on the bottleneck port $\ell_b$ (line $8$) which complete before their deadline if scheduled last on $\ell_b$. 
If $\mathcal{S}^d_{\ell_b}$ is not empty (Lines 10--13), it selects a coflow $k_n \in \mathcal{S}^d_{\ell_b}$ that has the largest deadline in $\mathcal{S}^d_{\ell_b}$. 
%------------------------------------------------------------------
% NOTE: Dans ce papier on n'utilise qu'une seule stratégie pour choisir k_n: Max Deadline !!!
% If such set is not empty, it selects a coflow $k_n$ among them using function $\mathtt{AdmittedCoflow}$. %This function is called if there are at least two coflows in $\mathcal{S}^d_{\ell_b}$. 
% This function selects the coflow with the lesser impact on the average CCT. We have considered three possible variants:
% \begin{itemize}
% \item Max Deadline ($\mathtt{DCoflow\text{-}MD}$): select the coflow with the largest deadline in $\mathcal{S}^d_{\ell_b}$. 
% \item Largest Processing Time (($\mathtt{DCoflow\text{-}LPT}$)): select the coflow with the largest processing time at bottleneck $\ell_b$ at $n$-th round.
% \item Ordering Coflow ($\mathtt{DCoflow\text{-}OC}$): identify a coflow ordering (e.g., according to the Sincronia algorithm  \cite{agarwal2018sincronia}) in $\mathcal{S}^d_{\ell_b}$ that minimizes the average CCT; the last coflow will be scheduled at the current round. 
% \end{itemize}
%------------------------------------------------------------------
%The second part of Algorithm~\ref{algo:DCoflow} (Lines 13--15)  introduces three variants, each of which corresponds to a different
%criterion to select the candidate coflow $k^{\star}$ that minimizes $\Psi_{\ell k}$, \textit{i.e}., the coflow that most likely violates
%the constraint \eqref{eq:fls_constraint_split}. 
If $\mathcal{S}^d_{\ell_b}$ is empty (Lines 14--18), i.e., no coflow respects its deadline when scheduled last on the bottleneck (Line $13$), the algorithm selects a coflow to be removed using function $\mathtt{RejectedCoflow}$, whose aim is to comply with parallel inequalities according to \eqref{eq:fls_constraint_split}. We consider two variants, each of which corresponds to a slightly different criterion to select the candidate coflow $k^{\star}$ by taking into account its weight. %hat minimizes $\Psi_{\ell k}$, \textit{i.e}., the coflow that most likely violates the constraint \eqref{eq:fls_constraint_split}. 

% The first variant, namely $\mathtt{DCoflow\_v1}$, finds the candidate $k^{\star}\in\mathcal{S}_{b}$ and \textit{every} link $\ell$ used by $k$,
% $$
% k^{\star}=\underset{k\in\mathcal{S}_{b},\ell:p_{\ell k}>0}{\mathrm{arg\,min}}\,w_k \Psi_{\ell k}.
% $$

The first variant, namely $\mathtt{DCoflow\_v1}$, 
finds the candidate $k^{\star}\in\mathcal{S}_{b}$ and every port $\ell$
used by $k$ where it fails to meet the deadline (that is, $\Psi_{\ell, k}<0$),
\begin{equation}
k^{\star}=\underset{k\in\mathcal{S}_{b}}{\mathrm{arg\,min}}\,{\displaystyle \Big( \sum_{\ell:\Psi_{\ell, k}<0}}\Psi_{\ell, k}\Big).
\end{equation}
The second variant, namely $\mathtt{DCoflow\_v2}$, finds
the candidate $k^{\star}\in\mathcal{S}_{b}$ and every port $\ell$
used by $k$ that has at least $\gamma$ times the congested level
of the bottleneck, \textit{i.e}., $\ell:\sum_{j}p_{\ell j}\geq\gamma\sum_{j}p_{bj}$,
\begin{equation}
k^{\star}=\underset{k\in\mathcal{S}_{b}}{\mathrm{arg\,min}}\,{\displaystyle \Big(  \sum_{\ell:\sum_{j}p_{\ell j}\geq\gamma\sum_{j}p_{bj}}}\Psi_{\ell k}\Big).
\end{equation}
Once the initial scheduling order $\sigma$ is obtained, $\mathtt{DCoflow}$ uses the function $\mathtt{RemoveLateCoflows}$ to estimate the CCT and remove from $\sigma$ the coflows that do not satisfy the deadline constraint (Line $20$). 
Briefly, $\mathtt{RemoveLateCoflows}$ considers each pre-rejected coflow $k^{\star}$ in $\sigma^{\star}$ (Line $24$). It calls the function $\mathtt{evalCCT}$ to evaluate the CCT of $k^{\star}$, given all the coflows in $\sigma$ that are scheduled before $k^{\star}$ (Line $25$). If $k^{\star}$ cannot meet its deadline, i.e., $c_{\sigma_{k^{\star}}} > T_{\sigma_{k^{\star}}}$, it will be removed permanently from $\sigma^{\star}$ and $\sigma$. $\mathtt{RemoveLateCoflows}$ performs a swipe on the admitted coflows (as in \cite{Luo2016}) and iteratively removes coflows in $\sigma$ that belong to $\sigma^{\star}$ until the estimated CCT $c_{\sigma_{k}}$ of each coflow $\sigma_{k} \in \sigma$ is of at most $T_{\sigma_{k}}$.

It is important to note that the final solution yielded by $\mathtt{DCoflow}$ does not guarantee all coflows in $\sigma$ to satisfy their deadlines. In Sec.~\ref{sec:Evaluation}, the prediction error of $\mathtt{DCoflow}$  indicates the gap between the estimated CAR and the actual CAR after applying resource allocation.  
% starts by calling the function $\mathtt{evalCCT()}$ to evaluate the CCT of all coflows in $\sigma$ (Line 3). Having this, the set of pre-rejected coflows $\sigma^{\star}$ is determined (Line 5). Finally, the coflows in $\sigma$ that belong to $\sigma^{\star}$ are sequentially removed from $\sigma$ until the estimated CCT $C_{\sigma_{k}}$ of each coflow in $\sigma$ is at most $T_{\sigma_{k}}$ (Lines 5--13). 


% \begin{table}
% \begin{center}
% \caption{Execution of $\mathtt{DCoflow}$ on the example of Fig.~\ref{fig:Example}. \label{tab:Example} }
% \begin{tabular}{|l|c|c|}
%   \hline
%  Unscheduled coflows  & Bottleneck & $\bar\Psi$ \\
%  (set $S$) & & $\{\bar\Psi_{1}, \bar\Psi_{2},\bar\Psi_{3},\bar\Psi_{4}\} $ \\
%   \hline
%  $ S=\{ \mathbf{C1}, \mathbf{C2}, C3, C4, C5\}$ & 1 & $\{-4(1+\varepsilon),-\varepsilon,*,*,* \} $\\
%     \hline
%   $S=\{ \mathbf{C2},C3, C4, C5\}$& 1& $\{*,0,*,*,*\}$  \\
%     \hline
%   $S=\{ \mathbf{C3}, C4, C5\}$ & 2 & $\{*,*,0,*,*\} $\\
%     \hline
%  $S=\{ \mathbf{C4}, C5\}$ & 3 & \{*,*,*,$0$,*\} \\
%      \hline
%  $S=\{ \mathbf{C5}\}$ & 4 & $\{*,*,*,*,0\}$ \\
%      \hline
% \end{tabular}
% \end{center}
% \end{table}



\vspace{0.2cm}
{\noindent\em Example.} 
To illustrate the difference between $\mathtt{DCoflow}$  and  $\mathtt{CS\text{-}MHA}$, we consider again the example  illustrated in Fig.~\ref{fig:Example}. Table \ref{tab:Example} shows the execution of $\mathtt{DCoflow\_v1}$ on that example. At the first step, $\mathtt{DCoflow\_v1}$ chooses bottleneck ingress port $1$, which is used by coflows $C_{1}$ and $C_{2}$. It computes $\overline{\Psi}_{ k} = \sum_{\ell:\Psi_{\ell, k} < 0 } \Psi_{\ell, k}$ for both coflows  and  selects the coflow with smallest $\bar\Psi_{ k}$ (in this case, $C_{1}$) to be scheduled last. Since all unscheduled coflows do not share any port in the fabric, any ordering of remaining coflows gives the same average CAR.  Given the final schedule, $\mathtt{DCoflow}$ obtains $\frac{4}{5}$  as the average CAR, which is the optimal solution.  


\begin{table}[t]
\caption{Execution of $\mathtt{DCoflow}$ on the example of Fig.~\ref{fig:Example}. \label{tab:Example}}
\centering
\begin{tabular}{
>{\raggedright}m{0.38\columnwidth}
>{\centering}p{0.05\columnwidth}
>{\centering}p{0.37\columnwidth}
}
\toprule 
Unscheduled coflows (set $\mathcal{S}$) & $\ell_{b}$ & 
$ \left\{ 
\overline{\Psi}_{1},
\overline{\Psi}_{2},
\overline{\Psi}_{3},
\overline{\Psi}_{4},
\overline{\Psi}_{5}
\right\} $ \tabularnewline
\cmidrule[0.4pt](lr{0.12em}){1-1}%
\cmidrule[0.4pt](lr{0.12em}){2-2}%
\cmidrule[0.4pt](lr{0.12em}){3-3}%
$\mathcal{S}=\left\{ \boldsymbol{C_{1}},\boldsymbol{C_{2}},C_{3},C_{4},C_{5}\right\} $ & 1 & $\left\{ -4\left(1+\varepsilon\right),-\varepsilon,\,\cdot\,,\,\cdot\,,\,\cdot\,\right\} $\tabularnewline
$\mathcal{S}=\left\{ \boldsymbol{C_{2}},C_{3},C_{4},C_{5}\right\} $ & 1 & $\left\{ \,\cdot\,,0,\,\cdot\,,\,\cdot\,,\,\cdot\,\right\} $\tabularnewline
$\mathcal{S}=\left\{ \boldsymbol{C_{3}},C_{4},C_{5}\right\} $ & 2 & $\left\{ \,\cdot\,,\,\cdot\,,0,\,\cdot\,,\,\cdot\,\right\} $\tabularnewline
$\mathcal{S}=\left\{ \boldsymbol{C_{4}},C_{5}\right\} $ & 3 & $\left\{ \,\cdot\,,\,\cdot\,,\,\cdot\,,0,\,\cdot\,\right\} $\tabularnewline
$\mathcal{S}=\left\{ \boldsymbol{C_{5}}\right\} $ & 4 & $\left\{ \,\cdot\,,\,\cdot\,,\,\cdot\,,\,\cdot\,,0\right\} $\tabularnewline
\bottomrule
\end{tabular}
\end{table}

\vspace{0.2cm}
{\noindent\em Online Implementation.}
\dcoflow\ can be also be run online, when coflows arrive sequentially and possibly in batches. For this, define $f$ to be the frequency of updates, i.e., instants at which \dcoflow\ recomputes a schedule. The updates can be performed either at arrival instants of coflows (in which case we set $f=\infty$) or periodically with period $1/f$. We assume that the scheduler knows the volumes of the flows of each arrived coflow. However, it neither knows the volumes nor the release times of future coflows. 

At each update instant, \dcoflow\ recomputes the scheduling order for coflows currently available in the network. These include the ones that were scheduled in the previous scheduling instants and have not yet finished; the ones that were rejected in the previous scheduling instants but whose deadline has not yet expired and the arrivals during the update interval. \dcoflow\ calculates the new order for this set of coflows based on the remaining volumes of the flows and not on the original volumes. Note that it is assumed that coflows can be preempted \cite{chowdhury2015coflow}. This process is repeated at each update instant.

\vspace{0.2cm}
{\noindent\em Complexity Analysis.} The complexity of $\mathtt{DCoflow}$ is $\cO(N^2)$. Specifically, in $\mathtt{DCoflow}$, the values $\sum_{i \in \cS} p_{\ell,i}$ and  $\Psi_{\ell, x}$ of each remaining coflow $x$ can be pre-stored by calculating them at a cost $\cO(NL)$, where $L = |\cL|$ is the number of ports. Then these  values can be updated at a cost $\cO(L)$ per coflow at each iteration. The number of operations required at Lines $11$--$13$ is $\cO(N)$ and at Lines $15$--$16$ is $\cO(N)$, so that finally across iterations it adds to $\cO(N^2)$. On the other hand, it is easy to verify the complexity of $\mathtt{RemoveLateCoflows}$ is  $\cO(NL)$. 




==> sections/Numerics-old.tex <==
% !TEX root = ../TPDCSW.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Performance Evaluation 
\label{sec:Evaluation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we evaluate our algorithms against state-of-the-art algorithms proposed in the literature.   In the interest of fairness and clarity, we  start  our evaluation by assigning the same weights to the coflows, as many algorithms are developed without the ability to \ob{handle different coflow weights}. In the second part  of this section, we treat the case with different  weights. 

% assign different weights to the coflows

%\vspace{-0.5cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulation Setup
\label{subsec:Simulation-Setup}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We evaluate via simulations our proposed heuristics (three variants:   $\mathtt{DCoflow}$\footnote{
The flow-level simulator and the implementation of all algorithms tested in this paper are available at https://github.com/luuquangtrung/CoflowSimulator.}, \wdcoflow \ and \wdcoflowDP) along with some existing algorithms such as $\mathtt{CS\text{-}MHA}$\footnote{
We only reimplemented the centralized algorithm ($\mathtt{CS\text{-}MHA}$) presented in \cite{Luo2016}, which has been reported to be better than the decentralized version ($\mathtt{D\textsuperscript{2}\text{-}CAS}$) in terms of CAR.
} 
and the solution provided by the optimization method $\mathtt{CDS\text{-}LP}$ proposed in \cite{Tseng2019}. The relaxed version of $\mathtt{CDS\text{-}LP}$, named $\mathtt{CDS\text{-}LPA}$, is also implemented\footnote{
It is worth noting that the formulation of $\mathtt{CDS\text{-}LP}$ and $\mathtt{CDS\text{-}LPA}$ use the same decision variables $\{z_k\}_{k \in \cC}$ as those introduced in Problem~\eqref{prob:CAR}. In $\mathtt{CDS\text{-}LP}$, $z_k$ are binaries, whereas in $\mathtt{CDS\text{-}LPA}$, $z_k$ are continuous variables taking values in $[0,1]$. For any solution yielded by $\mathtt{CDS\text{-}LPA}$, only coflows $k$ whose ${z_k}$ strictly equals $1$ are considered as accepted ones.
}. By using the solution derived from $\mathtt{CDS\text{-}LP}$ as an upper bound, we can get the sense of how close the algorithms are to the optimum. 
A brief description of the reference algorithms has been given in Sec.~\ref{sec:Introduction}. We also compare the performance of our schedulers against $\mathtt{Sincronia}$ \cite{Agarwal2018} and $\mathtt{Varys}$ \cite{Chowdhury2014} that aim to minimize the average CCT.  

Once we obtained the $\sigma$-order, the actual coflow resource allocation for our solution is implemented by the greedy rate allocation algorithm $\mathtt{GreedyFlowScheduling}$ \cite{Agarwal2018}.  At any given point of time, $\mathtt{GreedyFlowScheduling}$ reserves the full port bandwidth to one flow at the time. It does so by complying to the scheduling order in $\sigma$ of the coflow to which the flow belongs \cite{Agarwal2018}. We note that, in the case of $\mathtt{CDS\text{-}LP}$, $\mathtt{CDS\text{-}LPA}$, and $\mathtt{Varys}$, instead, the rate allocation is part of the algorithmic solution. 

The network fabric is represented by $M$ machines or end-hosts connected to a non-blocking Big-Switch fabric, of which each access port has a \textit{normalized} capacity of $1$. The algorithms will be evaluated on both small-scale and large-scale networks, where a network is denoted by $[M, N]$ to indicate different fabric size and number of coflows ($N$) used in the simulations. Small-scale networks have a fabric of size $M = 10$, whereas large-scale networks have a fabric with either $50$ or $100$ machines. The coflows in these networks are generated from both synthetic and real traffic traces.  

The MILP solver $\mathtt{gurobi}$ is used to solve $\mathtt{CDS\text{-}LP}$ and $\mathtt{CDS\text{-}LPA}$. Due to their high complexity, $\mathtt{CDS\text{-}LP}$ and $\mathtt{CDS\text{-}LPA}$ are only evaluated on small-scale networks. In what follows, the detailed setup, comparison metrics, and simulation results are presented.  

%%%%

\noindent{\em Synthetic Traffic traces}
The synthetic traffic comprises two types of coflows. Type-$1$ coflows have only one flow, whereas the number of flows of Type-$2$ coflows follows a uniform distribution in $[2M/3, M]$. Each generated coflow is randomly assigned to either Class $1$ or Class $2$ with probability of  $0.6$ and $0.4$, respectively. 
Moreover, each coflow $k$ is assigned a random deadline within $[\text{CCT}_k^0, \alpha \text{CCT}_k^0]$), where $\text{CCT}_k^0$ is the completion time of coflow  \emph{in isolation} and $\alpha$ a positive real  value with $2\leq \alpha \leq 4$.  A higher value of $\alpha$ means that the scheduler has more flexibility to meet the coflow deadline. 
% Flows of Class-$1$ coflows are assigned a random volume of mean of $1$ and standard deviation of $0.2$. The volume ratio for the flows of Class-$1$ and Class-$2$ coflows is $0.8$.


\vspace{0.2cm}
\noindent{\em Real Traffic traces}
Real traffic datasets are obtained by the Facebook traces dataset \cite{Chowdhury2014}, based on a MapReduce shuffle trace collected from one of Facebook's $3000$-machine cluster with $150$ racks. The data traces consist of $526$ coflows. They have a skewed coflow width distribution, ranging from coflows with a single flow to very large ones (the largest coflow has $21170$ flows). For detailed statistics of the Facebook traces we refer the reader to \cite{ChowdhuryThesis2015}. For each configuration $[M,N]$, $N$ coflows are randomly sampled from the Facebook dataset. Coflows are only selected from the ones that have at most $M$ flows. The volume of each flow is given by the dataset. 

\vspace{0.2cm}
\noindent{\em Weight Classes.} 
For \wdcoflow\ and \wdcoflowDP\ we consider two  classes of weights for both synthetic and real traffic. The weight of each coflow reflects its level of importance. Class-$1$ coflows are assigned a weight $w_1 = 1$ and Class-$2$ coflows are assigned a weight $w_2$ of either $2$ or $10$. The probability that each generated coflow falls into Class $1$ and Class $2$ are respectively $p_1$ and $p_2 = 1-p_1$. 


\vspace{0.2cm}
\noindent{\em Metric.}
%Two metrics are used for algorithm comparison: 
\ob{
We evaluate the algorithms based on the average weighted coflow acceptance rate $\text{WCAR} = \frac{\sum_{k \in \cC} w_k z_k}{\sum_{k \in \cC} w_k}$. In the unweighted setting, WCAR is just the average CAR. We also present  the gains in percentiles of each algorithm with respect to the solution yielded by $\mathtt{CDS\text{-}LP}$ in terms of WCAR. These gains are calculated using the formula: $\text{average gain in WCAR} = \frac{\text{compared WCAR}}{\text{WCAR under } \mathtt{CDS\text{-}LP}} - 1.$
}
%We evaluate the algorithms based on the average CAR. We also present  the gains in percentiles of each algorithm with respect to the solution yielded by $\mathtt{CDS\text{-}LP}$ in terms of CAR. These gains are calculated using the formula: $\text{average gain in CAR} = \frac{\text{compared CAR}}{\text{CAR under } \mathtt{CDS\text{-}LP}} - 1.$

%Although, the main metric is average CAR, we also compared the average CCTs of the algorithms. Due to lack of space, we shall mention only briefly the main findings and not any figures.

% \eqref{eq:PR:Rate}.
% \begin{equation}\label{eq:PR:Rate}
% \text{avg. gain in CAR} = \frac{\text{compared CAR}}{\text{CAR under } \mathtt{CDS\text{-}LP}} - 1.
% \end{equation}

% \vspace{-0.2cm}
% {
% \begin{align}
% \text{avg. gain in CAR} & = \frac{\text{compared CAR}}{\text{CAR under } \mathtt{CDS\text{-}LP}} - 1 \label{eq:PR:Rate}
% % \text{avg. gain in norm. CCT} & = 1 - \frac{\text{compared norm. CCT}}{\text{norm. CCT under } \mathtt{CDS\text{-}LP}} \label{eq:PR:CctNorm}
% \end{align}
% }

\subsection{Unweighted scheduling coflows}
In this section,  we evaluate our algorithm against the other  algorithms described in section~\ref{subsec:Simulation-Setup}  when the same weights are assigned to all coflows.  We recall that the unweighted case represents the evaluation of $\mathtt{DCoflow}$  initially developed in \cite{Dcoflow22}. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Results with Offline Setting  \label{sec:Eva:Offline}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $\mathtt{DCoflow\_v1}$
% $\mathtt{DCoflow\_v2}$
% $\mathtt{DCoflow\_v3}$
% $\mathtt{Sincronia}$
% $\mathtt{Varys}$
% $\mathtt{CS\text{-}MHA}$
% $\mathtt{CDS\text{-}LP}$
% $\mathtt{CDS\text{-}LPA}$

In the offline setting, we consider that all coflows arrive at the same time, i.e., their release time is zero. For each simulation with a specific scale of the network and either synthetic or real traffic traces, we randomly generate $100$ different instances and compute the average performance of algorithms over $100$ runs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{{Average CAR Under Synthetic Traffic}}\label{sec:Eva:Offline:Rd}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figs.~\ref{fig:Off:Rate:Random:Small}--\ref{fig:Off:Rate:Random:Big} show the average CAR with respectively small-scale networks and large-scale networks. The percentile gains of each algorithm with respect to $\mathtt{CDS\text{-}LP}$  are shown in Fig.~\ref{fig:Off:Percentile:Random}, in terms of average CAR for the configuration $[10,60]$.


%--------------------------------------------------------------------------
% GENERATED TRACE - ACCEPT RATE
\begin{figure}[h]
\centering
% low workload
\subfloat[{Synthetic traffic
traces on a small-scale network.\label{fig:Off:Rate:Random:Small} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_rate_rd_small.pdf}}

\vspace{-0.2cm}

% high workload
\subfloat[{Synthetic traffic
traces on a large-scale network.\label{fig:Off:Rate:Random:Big} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_rate_rd_big.pdf}}
\caption{Average CAR with synthetic traffic traces using (a) small-scale and (b) large-scale networks. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Rate:Random}}
%\vspace{-0.5cm}
\end{figure}



% GENERATED TRACE - PERCENTILE OF GAINS WITH LOW WORKLOADS
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.492\columnwidth]{fig_coflow/results/offline/off_comp_rac_Pr_rd_M10_C60.pdf}
%\caption{The $1$\textsuperscript{st}-$10$\textsuperscript{th} -$50$\textsuperscript{th}-$90$\textsuperscript{th}-$99$\textsuperscript{th} percentiles of the average gain in CAR using synthetic traces with workload $[10,60]$.  \label{fig:Off:Percentile:Random}}
%\end{figure}
%--------------------------------------------------------------------------



It is observed that \dcoflow \  is closest in terms of CAR to the optimum ($\mathtt{CDS\text{-}LP}$) than all other algorithms, with both small- and large-scale networks,  and even outperforms $\mathtt{CDS\text{-}LPA}$, the approximation version of $\mathtt{CDS\text{-}LP}$. 
For instance, on the network $[10,10]$, $\mathtt{DCoflow}$ improves the CAR on average by 
$6.5\%$,
$11.5\%$,
$15.1\%$, and
$26.6\%$,
compared respectively to 
$\mathtt{CDS\text{-}LPA}$, 
$\mathtt{CS\text{-}MHA}$,
$\mathtt{Sincronia}$, and
$\mathtt{Varys}$. 
Interestingly, the improvement becomes higher when the load is increased. For example, the corresponding improvement on average CAR on a $[10,60]$ network are 
$67.2\%$,
$98.3\%$,
$59.9\%$, and
$36.8\%$ 
(see Fig.~\ref{fig:Off:Rate:Random:Small}). The improvement is even higher when performed on a large-scale network. For example, compared to 
$\mathtt{CS\text{-}MHA}$,
$\mathtt{Sincronia}$, and
$\mathtt{Varys}$, on the network $[100,400]$, the improvement in terms of average CAR are respectively
$648.1\%$,
$32.3\%$, and
$17.9\%$.
(see Fig.~\ref{fig:Off:Rate:Random:Big}). It is worth noting how the performance of $\mathtt{CS\text{-}MHA}$ falls drastically when dealing with large-scale networks.
This is expected since  $\mathtt{CS\text{-}MHA}$ prioritizes coflows that use a large number of ports over those that use a few. In instances with a large number of coflows of the latter type, the CAR of $\mathtt{CS\text{-}MHA}$ goes to $0$ (see detailed explanation with the motivating example in Sec.~\ref{subsec:Motivating-Example})

%cannot make the difference between a coflow with large number of flows and a large number of coflows with a single flow (see motivated example in Sec.~\ref{subsec:Motivating-Example}).
%Indeed $\mathtt{CS\text{-}MHA}$  can make an arbitrary scheduling since the impact is measured at each port without taking into account the relative impact due to conflicting volumes over multiple ports. 
%This happens when the set of coflows involved in a port is different on other ports; therefore, an admitted coflow that uses several ports, could make the scheduler refuse several coflows that have a later deadline.
%since their deadline cannot be met if it is scheduled before them.   

The result in Fig.~\ref{fig:Off:Percentile:Random} shows that $\mathtt{DCoflow}$ achieves a smaller gap to the optimal in almost all values of percentile compared to other algorithms. For instance, compared to $\mathtt{Sincronia}$, $\mathtt{DCoflow}$ improves the CAR in $50\%$ of $100$ instances by $50\%$ and it achieves around $43\%$ at $99$\textsuperscript{th} percentile. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Average CAR Under Real Traffic Traces}\label{sec:Eva:Offline:Fb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section presents the results obtained with the Facebook traffic traces, using the same configurations as those used in Sec.~\ref{sec:Eva:Offline:Rd}. Figs.~\ref{fig:Off:Rate:Facebook:Small}--\ref{fig:Off:Rate:Facebook:Big} show the average CAR with respectively small- and large-scale networks. The gains in percentiles of each algorithm with respect to $\mathtt{CDS\text{-}LP}$, in terms of average CAR when using a $[10,60]$ fabric are shown in Fig.~\ref{fig:Off:Percentile:Facebook}. Similar to what observed in the results with the synthetic traces (see Sec.~\ref{sec:Eva:Offline:Rd}), $\mathtt{DCoflow\_v1}$ and $\mathtt{DCoflow\_v2}$ yield a significant improvement in terms of average CAR compared to other heuristics. For instance, with a $[10,60]$ configuration, the two variants of $\mathtt{DCoflow}$ improve the average CAR on average by  
$24.4\%$,
$25\%$,
$52.2\%$,
$93.1\%$,
compared respectively to 
$\mathtt{CDS\text{-}LPA}$, 
$\mathtt{CS\text{-}MHA}$,
$\mathtt{Sincronia}$, and
$\mathtt{Varys}$.
(see Fig.~\ref{fig:Off:Rate:Facebook:Small}). The improvement is even higher when performed on a large-scale network. For example, compared to 
$\mathtt{CS\text{-}MHA}$,
$\mathtt{Sincronia}$, and
$\mathtt{Varys}$, on $[100,400]$ network, the improvement in terms of average CAR are respectively
$36.6\%$,
$55.3\%$, and
$147.5\%$.

Moreover, the results in Fig.~\ref{fig:Off:Percentile:Facebook} show that the two variants of $\mathtt{DCoflow}$ achieve a smaller gap to the optimal in almost all values of percentile compared to the other algorithms. 
For instance, compared to $\mathtt{Sincronia}$, $\mathtt{DCoflow\_v1}$ improves the CAR in $57\%$ of $100$ instances by $50\%$ and it achieves around $35\%$ at $99$\textsuperscript{th} percentile. 

\begin{figure}[t]
\centering
% low workload
\subfloat[{Facebook traffic traces on a small-scale network.\label{fig:Off:Rate:Facebook:Small} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_rate_fb_small.pdf}}

\vspace{-0.2cm}

% high workload
\subfloat[{Facebook traffic traces on a large-scale network.\label{fig:Off:Rate:Facebook:Big} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_rate_fb_big.pdf}}
\caption{Average CAR with Facebook traces using (a) small-scale network and (b) large-scale network. Each point in the x-axis represents network $[M,N]$. \label{fig:Off:Rate:Facebook}}
\end{figure}

% FACEBOOK TRACE - GAINS
\begin{figure}[t]
\centering
% Random
\subfloat[{Synthetic traces. \label{fig:Off:Percentile:Random}}]{
\includegraphics[width=0.4\columnwidth]{fig_coflow/results/offline/off_comp_rac_Pr_rd_M10_C60.pdf}}
% Facebook
% \vspace{-0.3cm}
\subfloat[{Facebook traces.\label{fig:Off:Percentile:Facebook} }]{
\includegraphics[width=0.4\columnwidth]{fig_coflow/results/offline/off_comp_rac_Pr_fb_M10_C60.pdf}}
\caption{The $1$\textsuperscript{st}-$10$\textsuperscript{th} -$50$\textsuperscript{th}-$90$\textsuperscript{th}-$99$\textsuperscript{th} percentiles of the average gain in CAR with small-scale network $[10,60]$ using (a) synthetic and (b) Facebook traces. \label{fig:Off:Percentile}}
\vspace{-0.5cm}
\end{figure}
 %--------------------------------------------------------------------------




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Prediction Error of $\mathtt{DCoflow}$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As mentioned at the end of Sec.~\ref{sec:heuristic}, we also evaluate the prediction error $(|\sigma| - |\hat{\sigma}|)/|\sigma|$ of our heuristics, where $\hat{\sigma} \subseteq \sigma$ is the set of coflows in $\sigma$ that satisfy the deadline constraint after performing the actual resource allocation using $\mathtt{GreedyFlowScheduling}$. Both variants of $\mathtt{DCoflow}$ provide a prediction of CAR with an average error below $3.6\%$ for both traffic traces. 


\begin{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Comparison of average CCT} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As mentioned previously, due to lack of space we present only a brief comparison of the average CCTs. On small-scale networks the he his actually shows a relatively good performance of $\mathtt{DCoflow}$ in terms of minimizing the average CCT, though it is not the main objective of our proposed heuristics.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Average Normalized CCT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Fig.~\ref{fig:Off:Cct:Random} and \ref{fig:Off:Cct:Facebook} show respectively the average normalized CCT of accepted coflows using synthetic and Facebook traces. 
As $\mathtt{DCoflow}$ is able to accept more coflows (see Sec.~\ref{sec:Eva:Offline:Rd} and \ref{sec:Eva:Offline:Fb}), as a consequence, the average normalized CCTs yielded by $\mathtt{DCoflow\_v1}$ and $\mathtt{DCoflow\_v2}$ are slightly higher than that of other algorithms, as shown in Figs.~\ref{fig:Off:Cct:Random} and \ref{fig:Off:Cct:Facebook}. This actually shows a relatively good performance of $\mathtt{DCoflow}$ in terms of minimizing the average CCT, though it is not the main objective of our proposed heuristics.



%--------------------------------------------------------------------------
% RANDOM & FACEBOOK TRACE - ACCEPT NORMALIZED CCT
\begin{figure}[t]
\centering
% low workload
\subfloat[{Synthetic traces.\label{fig:Off:Cct:Random} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_cct_rd_small.pdf}}

% high workload
\subfloat[{Facebook traces.\label{fig:Off:Cct:Facebook} }]{
\includegraphics[width=.7\columnwidth]{fig_coflow/results/offline/off_cct_fb_small.pdf}}
\caption{Average normalized CCT using small-scale networks with (a) synthetic and (b) Facebook traces. Each point in the x-axis represents network $[M,N]$. \label{fig:Off:Cct}}
\end{figure}
%--------------------------------------------------------------------------



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computing Time}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The average processing time per instance for the \textit{scheduling} phase of the all algorithms with the Facebook traces is reported in Table~\ref{tab:Eva:Time}. The value in parentheses is the total time elapsed for the scheduling phase (only applicable for $\mathtt{DCoflow}$, $\mathtt{Sincronia}$ and $\mathtt{CS\text{-}MHA}$). It is observed that $\mathtt{DCoflow}$ requires more time for scheduling than other heuristics. Nevertheless, by using $\mathtt{RemoveLateCoflows}$ to remove (expectedly) late coflows from the order $\sigma$, $\mathtt{DCoflow}$ needs lesser time to finish both scheduling and resource allocation. On the other hand, as expected, due to high complexity, $\mathtt{CDS\text{-}LPA}$ and $\mathtt{CDS\text{-}LP}$ consume more time than other algorithms, and the time consumption of these methods grows exponentially with the increase of the network scale.

%--------------------------------------------------------------------------
\begin{table}[h]
\caption{Processing Time with Facebook Traces (s). \label{tab:Eva:Time}}
\scriptsize
\centering{}%
\begin{tabular}{
>{\raggedright}p{0.15\columnwidth}
>{\centering}p{0.25\columnwidth}
>{\centering}p{0.25\columnwidth}
}
\toprule 
Methods & Network $[10,60]$ & Network $[100,400]$\tabularnewline
\cmidrule[0.4pt](lr{0.12em}){1-1}%
\cmidrule[0.4pt](lr{0.12em}){2-2}%
\cmidrule[0.4pt](lr{0.12em}){3-3}%
$\mathtt{CDS\text{-}LP}$ & --- (21.8) & ---\tabularnewline
$\mathtt{CDS\text{-}LPA}$ & --- (12.8) & ---\tabularnewline
$\mathtt{CS\text{-}MHA}$ & 0.01 (0.189) & 0.07 (42.4)\tabularnewline
$\mathtt{DCoflow\_v1}$ & 0.027 (0.075) & 5.31 (9.81)\tabularnewline
$\mathtt{DCoflow\_v2}$ & 0.027 (0.077) & 5.32 (9.79)\tabularnewline
$\mathtt{Sincronia}$ & 0.016 (0.118) & 0.58 (14.9)\tabularnewline
$\mathtt{Varys}$ & --- (0.9) & --- (20.5)\tabularnewline
\bottomrule
\end{tabular}
\end{table}
%--------------------------------------------------------------------------
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Online Setting 
\label{sec:Eva:Online}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now present a series of numerical results on the performance of the online version of $\mathtt{DCoflow}$. The metric used for the performance evaluation is the average CAR obtained over $40$ instances. In each instance, coflows arrive sequentially according to a Poisson process of rate $\lambda$, i.e., the inter-arrival time of coflows is exponentially distributed with rate $\lambda$. Unless stated otherwise, %we assume that coflow priorities (that is, the order in which they are processed) are computed  upon arrival of a new coflow ($f=\infty$). 
coflow priorities %(that is, the order in which they are processed) 
are computed  upon arrival of a new coflow ($f=\infty$). 
% Recall that coflow priorities (that is, the order in which they are processed) can be computed either upon arrival of a new coflow ($f=\infty$), or at fixed interval of times of length $\frac{1}{f}$. 
%We assume that the schedulers are aware of the volume of flows in the arriving coflow but not the future demand. It is also assumed that the transport layer allocates resources to coflows according to the greedy algorithm.


As both versions of $\mathtt{DCoflow}$ provide similar results, we only present the results obtained with $\mathtt{DCoflow\_v1}$. The average CAR obtained with $\mathtt{DCoflow\_v1}$ is compared against those obtained with the online version of Varys with deadline \cite{Ma2016}, $\mathtt{CS\text{-}MHA}$ and $\mathtt{Sincronia}$. We investigate the effect of two main parameters: (\textit{i}) the coflow arrival rate $\lambda$ and (\textit{ii}) the frequency $f$ at which coflow priorities are updated.

%Those results are obtained on instances generated using our workload generator. We assess the performance of our algorithms against the online version of Varys with deadline \cite{}, $\mathtt{CS\text{-}MHA}$ and Sincronia. Coflow arrivals follow a Poisson process with an average rate of $\lambda$ coflows/slot. For each scheduling algorithm at each input load (obtained by varying \lqt{???}), we simulate 5000 coflow arrivals to get the average accepting rate  of all completed coflows. For the sake of comparison, we have used the greedy algorithm for resource  allocation.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Impact of Arrival Rate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We first study the impact of the arrival rate $\lambda$ on the CAR obtained with the various algorithms. The CAR is averaged over $40$ instances, each one with $4000$ coflow arrivals. % 
%Coflow arrival times follow a Poisson process with rate $\lambda$, 
The deadline of a coflow $k$ is drawn from a uniform distribution in $[\text{CCT}_k^0, 4\text{CCT}_k^0]$. We also consider two scenarios: a small fabric with $M = 10$ machines, and a large fabric with $M = 50$ machines. For each scenario, results are presented for the following values of $\lambda$: $\lambda = 8$, $\lambda = 12$, $\lambda = 16$, and $\lambda = 20$. 

Our results are shown in Figs.~\ref{fig:On:Rate:Random:Rachid:M10} and \ref{fig:On:Rate:Random:Rachid:M50}, for the small fabric scenario and the large one, respectively. We observe that $\mathtt{DCoflow\_v1}$ achieves a higher average CAR for all values of $\lambda$, and that the gain with respect to the other scheduling algorithms increases with the value of $\lambda$. If all algorithms achieve more or less the same CAR for a lightly loaded fabric, $\mathtt{DCoflow\_v1}$ clearly outperforms the other algorithms when the fabric is highly congested.

% RACHID's RESULT - [10,4000] and [50,4000], b = 4, lambda = [8,12,16,20]
\begin{figure}[t]
\centering
% low workload
\subfloat[{Small fabric.\label{fig:On:Rate:Random:Rachid:M10} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_rachid_random_m10_c4000_b4.pdf}}
% high workload
\subfloat[{Large fabric.\label{fig:On:Rate:Random:Rachid:M50} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_rachid_random_m50_c4000_b4.pdf}}
\caption{Average CAR using synthetic traffic with varying $\lambda$ and (a) $M = 10$ and (b) $M = 50$. \label{fig:On:Rate:Random:Rachid}}
\end{figure}


Figs.~\ref{fig:On:Rate:Facebook:Rachid:M10C4000F60} and \ref{fig:On:Rate:Facebook:Rachid:M100C4000F200} show respectively the average CAR obtained with $M=10$ and $M=100$, both with $4000$ coflows, using the Facebook dataset. Similar to what obtained with the synthetic traffic traces, $\mathtt{DCoflow\_v1}$ outperforms all other methods with significant gains. When the fabric is highly congested (i.e., with $M=10$), again $\mathtt{DCoflow\_v1}$ yields a higher gain compared to other algorithms. For instance, $\mathtt{DCoflow\_v1}$ achieves $9.3\%$ higher CAR than $\mathtt{Sincronia}$ when $M=100$ (see Fig.~\ref{fig:On:Rate:Facebook:Rachid:M100C4000F200}), while with $M=10$, the gap becomes $16.4\%$ (see Fig.~\ref{fig:On:Rate:Facebook:Rachid:M10C4000F60}).

% RACHID's RESULT - [10,4000] and [50,4000], b = 4, lambda = [8,12,16,20]
\begin{figure}[htb]
\centering
% low workload
\subfloat[{Small fabric.\label{fig:On:Rate:Facebook:Rachid:M10C4000F60} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_rachid_facebook_m10_c4000_b4_f60.pdf}}
% high workload
\subfloat[{Large fabric.\label{fig:On:Rate:Facebook:Rachid:M100C4000F200} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_rachid_facebook_m100_c4000_b4_f200.pdf}}
\caption{Average CAR using Facebook traffic with varying $\lambda$ and (a) $M = 10$ and (b) $M = 100$. \label{fig:On:Rate:Facebook:Rachid}}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Impact of Update Frequency}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As mentioned above, two different schemes can be envisioned for the update of coflow priorities. A first scheme is to update coflow priorities at periodic points in time, that is, every $\frac{1}{f}$ units of time. We refer to this scheme as the periodic update scheme with frequency $f$. As the update frequency $f$ and the coflow arrival rate should preferably be correlated, we consider the following values of $f$: $f=\frac{\lambda}{2}$, $f=\lambda$, and $f=2\lambda$. Another scheme is to update coflow priorities upon arrival of a new coflow. We refer to the latter scheme as the scheme with infinite frequency ($f=\infty$).

We now evaluate the impact of the update frequency $f$ on the average CAR. We consider the following values of $f$: $f=\frac{\lambda}{2}$, $f=\lambda$, $f=2\lambda$, and $f=\infty$. Recall that $f=\infty$ means that priorities are updated upon each coflow arrival. We assume that $M=10$ and compute the CAR by averaging over $40$ instances. For each instance, we simulate $8,000$ coflow arrivals according to a Poisson process at rate $\lambda$, assuming that the deadline of a coflow $k$ is uniformly distributed in $[\text{CCT}_k^0, 2\text{CCT}_k^0]$. We present the average CAR obtained for different values of $f$ ($f \in \{ \frac{\lambda}{2}, \lambda, 2\lambda,  \infty \}$) and for different values of the arrival rate $\lambda$ (from $2$ to $10$).

%For simplicity, we only compare $\mathtt{DCoflow\_v1}$ to $\mathtt{CS\text{-}MHA}$. Our results are shown in Fig.~\ref{fig:On:Rate:Random:Olivier}. 



% \vspace{-0.5cm}

% OLIVIER's RESULT - [10,8000], batch and no batch
\begin{figure}[t]
\centering
% low workload
\subfloat[{Without batch.\label{fig:On:Rate:Random:Olivier:nobatch} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_olivier_random_m10_c8000_nobatch.pdf}}
% high workload
\subfloat[{With batch.\label{fig:On:Rate:Random:Olivier:batch} }]{
\includegraphics[width=.49\columnwidth]{fig_coflow/results/online/on_olivier_random_m10_c8000_batch.pdf}}
\caption{Average CAR of $\mathtt{DCoflow\_v1}$ and $\mathtt{CS\text{-}MHA}$ using synthetic traffic with $[10,8000]$ and varying $\lambda$, when obtaining (a) one single coflow per arrival; and (b) a random batch of coflow per arrival. \label{fig:On:Rate:Random:Olivier}}
\end{figure}


The results in Fig.~\ref{fig:On:Rate:Random:Olivier:nobatch} are obtained from a simulation, in which each arrival corresponds to one single coflow. We note, as before, that for a low arrival rate, both algorithms provide a similar average CAR (for $\lambda=2$, $\mathtt{CS\text{-}MHA}$ achieves a slightly higher CAR than $\mathtt{DCoflow\_v1}$), but that $\mathtt{DCoflow\_v1}$ clearly outperforms $\mathtt{CS\text{-}MHA}$ when the fabric is highly congested. We also note that a higher frequency $f$ significantly improves the CAR for both algorithms. For instance, for $\lambda=2$ (resp. $\lambda=10$), the average CAR is increased by $52\%$ (resp. $46\%$) if we update coflow priorities upon arrival of each new coflow instead of using the periodic scheme with $f=\frac{\lambda}{2}$. These results suggest that there is a need for a trade-off between the computational complexity of updating coflow priorities at a high frequency and the CAR achieved.
In Fig.~\ref{fig:On:Rate:Random:Olivier:batch}, we present a similar result, but assuming that coflows arrive in batches. The batch size follows a uniform distribution $\mathcal{U}([5,15])$. Since the average number of coflows in each batch is $10$, in this setting, we divide the batch arrival rate by $10$ to obtain the same coflow arrival rates as in Fig.~\ref{fig:On:Rate:Random:Olivier:nobatch}. The results obtained for batch arrivals are similar to those obtained previously, but we note that the gains of $\mathtt{DCoflow\_v1}$ with respect to $\mathtt{CS\text{-}MHA}$ are significantly higher in this case. Moreover, we note that the benefit of using a higher update frequency is lower in this case (e.g., for $\lambda=10$, the average CAR is increased only by $17\%$ if we use $f=\infty$ instead of $f=\frac{\lambda}{2}$).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%Weighted scheduling coflows%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Weighted scheduling coflows}

In this section, we  now evaluate our proposed heuristic  \wdcoflow\ and \wdcoflowDP\ along with \csdp, \cdslp, and \cdslpa. \csdp\ is the adapted version to the weights of \csmha\ presented in \cite{Luo2016}, whereas \cdslp\ and its relaxed variant, \cdslpa, are the adapted to include the weights in the optimization methods introduced in \cite{Tseng2019} for the unweighted case. By using the solution derived from \cdslp\ as an upper bound, we would get the sense of how close the algorithms are to the optimum. 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Offline Setting  \label{sec:Eva:Off}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the offline setting, we consider that all coflows arrive at the same time, i.e., their release time is zero. For each simulation with a specific scale of the network and either synthetic or real traffic traces, we randomly generate $100$ different instances and compute the average performance of algorithms over $100$ runs. We  evaluate  \wdcoflow\ and \wdcoflowDP\ against  existing algorithms for the offline case. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Synthetic Traffic 
\label{sec:Eva:Off:Syn}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Figs.~\ref{fig:Off:Syn:WCAR:Small} and \ref{fig:Off:Syn:WCAR:Big} shows the average WCAR with synthetic traffic traces using small-scale ($M = 10$) and large-scale ($M = 100$) networks.  It is observed that our proposed heuristics (\wdcoflow\ and \wdcoflowDP)  are closest in terms of WCAR to the optimum (\cdslp) than all other algorithms in both small- and large-scale network configurations. \wdcoflowDP\  yields a slightly higher performance compared to \wdcoflow\ (around $4.2\%$) when using large-scale network settings (see Fig.~\ref{fig:Off:Syn:WCAR:Big}).  For small scale network,  we observe that  the optimum \cdslp obtain only a  gain of 9\%  and 7\% compared to   \wdcoflow\ and \wdcoflowDP\   respectively for $N=10$ .    On the other hand, CDS-LPA and CS-DP are far from the optimal solution by 17\% and 30\% respectively.  For the worst case when $N=60$,   \wdcoflow\ and \wdcoflowDP\   are far from the optimal solution by 19\% and 17\% respectively, but CDS-LPA and CS-DP moves away from the optimum by 42\% and 58\% respectively. 

Now, for large-scale networks, we observe that  \wdcoflow\ and \wdcoflowDP\  obtain significant performance compared to \csdp\. Indeed, for $N=100$,  \wdcoflow\ and \wdcoflowDP\  obtain a gain of 14\% and 18\% respectively.  When the number of coflows increases, both algorithms obtain gains up to 184\% for \wdcoflow\  and 192\% for \wdcoflowDP\  compared to  \csdp\ .


\begin{figure}[t]
\centering
\subfloat[{Small-scale networks.\label{fig:Off:Syn:WCAR:Small} }]
{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m10_p2_w2_wcar.pdf}
}
\subfloat[{Large-scale networks.\label{fig:Off:Syn:WCAR:Big} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m100_p2_w2_wcar.pdf}}
\caption{Average WCAR with coflows of all classes using synthetic traffic traces and (a) small-scale and (b) large-scale networks. The values of $(p_2,w_2)$ are set to $(0.2,2)$. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Syn:WCAR}}
\end{figure}



\begin{figure}[t]
\centering
\subfloat[{Small-scale networks.\label{fig:Off:Syn:WCAR:Small} }]
{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m10_p2_w2_wcar.pdf}
}
\subfloat[{Large-scale networks.\label{fig:Off:Syn:WCAR:Big} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m100_p2_w2_wcar.pdf}}
\caption{Average WCAR with coflows of all classes using synthetic traffic traces and (a) small-scale and (b) large-scale networks. The values of $(p_2,w_2)$ are set to $(0.2,2)$. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Syn:WCAR}}
\end{figure}

With respect to the performance of each class,
Figs.~\ref{fig:Off:Syn:ClassCAR:Small} and \ref{fig:Off:Syn:ClassCAR:Big} show the average WCAR of each coflow class  using small and large-scale networks.   As expected, the performance is even more significant for traffic of Class 2  since  \wdcoflow\ and \wdcoflowDP\ consider both the network conditions and coflows' importance  to perform the scheduling, while \csdp\  computes prioritizes coflows that use a large number of ports over those use a few.  Fig.~\ref{fig:Off:Syn:ClassCAR:Big}, we can see that  \wdcoflow\ and \wdcoflowDP\ perform about $21\%$ and $51\%$ for $N=100$ and $247\%$ and $258\%$ for $N=600$ better than \csdp\  for Class 2. 
For class 1 coflows, our heuristic achieves a moderate gain of up to 10\% for $N=600$ compared to \csdp\ .

\begin{figure}[t]
\centering
\subfloat[{Small-scale networks.\label{fig:Off:Syn:ClassCAR:Small} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m10_p5_w2_classcar.pdf}}
\subfloat[{Large-scale networks.\label{fig:Off:Syn:ClassCAR:Big} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m100_p5_w2_classcar.pdf}}
\caption{Average per-class CAR with synthetic traffic traces using (a) small-scale and (b) large-scale networks. The value of $p_2$ is set to $0.2$. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Syn:ClassCAR}}
\end{figure}


Figs.~\ref{fig:Off:Syn:ChangeParam:p2} and \ref{fig:Off:Syn:ChangeParam:w2} illustrate respectively the per-class WCAR with synthetic traffic traces using network configuration $[10,60]$ when varying $p_2$ (with fixed $w_2$) and $w_2$ (with fixed $p_2$).   We can see that both schedulers  \wdcoflow\ and \wdcoflowDP\  obtain almost the same performance compared to the optimal solution and they handle the priority between classes as \cdslp.  But for  Class 1, we can see that \csdp\ performs best for  $p_2=0.5$ and $p_2=0.8$.  This means that  \wdcoflow\ and \wdcoflowDP\  take  into account the importance of weight on how to schedule  the coflows.


\begin{figure}[t]
\centering
\subfloat[{Varying $p_2$ with fixed $w_2$.\label{fig:Off:Syn:ChangeParam:p2} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m10_c60_w2_changeP.pdf}}
\subfloat[{Varying $w_2$ with fixed $p_2$.\label{fig:Off:Syn:ChangeParam:w2} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_syn_m10_c60_p2_changeW.pdf}}
\caption{Average per-class CAR with synthetic traffic traces using network configuration $[10,60]$ when (a) varying $p_2$ with fixed $w_2 = 2$ and (b) varying $w_2$ with fixed $p_2 = 0.2$. \label{fig:Off:Syn:ChangeParam}}
\end{figure}

% \vspace{-0.5cm}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Real Traffic Traces}\label{sec:Eva:Off:Fb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% In this section, we use traces of Facebook to test the performance of \wdcoflow\ and \wdcoflowDP. As the original Facebook trace doesn't include weight information, we set random weights in $\{1,2\}$ to represent the importance of coflows. Here the  weight  $w_2=2$  is assigned to a coflow with probability $p_2$.
% NOTE: Cette introduction des poids sont dj mise dans la section 6.1 (Simulation Setup)

Now we use traces of Facebook to evaluate  the performance of \wdcoflow\ and \wdcoflowDP. 

Figs.~\ref{fig:Off:Fb:WCAR:Small} and \ref{fig:Off:Fb:WCAR:Big} show the average WCAR with Facebook traffic traces using small and large-scale networks.  The figures show that  \wdcoflow\ and \wdcoflowDP are closed to the optimal solution (the difference is less than 3\%) while CDS-LPA and CS-DP are far from the optimum of 5\% and 8\% respectively.   For high load (N=60), \wdcoflow\ and \wdcoflowDP lose only 10\% and 15\% respectively  compared to the optimal but the other two algorithms lose more ground by about 53\% compared to the optimal. 
Moreover, the performance gap becomes higher with the increase of the network scale. For instance, with network $[100,100]$, \wdcoflow\ and \wdcoflowDP\ perform around $6.8\%$ and $8.4\%$ better than \csdp\, while with the network $[100,600]$, these gaps become $20\%$ and $22\%$, respectively.





We observe that  \wdcoflow\ and \wdcoflowDP\ approximate the performance of the optimal solution for the small-scale network and perform better than \csdp\ on maximizing the average WCAR. Moreover, the performance gap becomes higher with the increase of the network scale. For instance, with network $[100,100]$, \wdcoflow\ and \wdcoflowDP\ perform around $10\%$ and $13\%$ better than \csdp\, while with the network $[100,600]$, these gaps become $331\%$ and $345\%$, respectively.

\begin{figure}[h]
\centering
\subfloat[{Small-scale networks.\label{fig:Off:Fb:WCAR:Small} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_fb_m10_p2_w2_wcar.pdf}}
\subfloat[{Large-scale networks.\label{fig:Off:Fb:WCAR:Big} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_fb_m100_p2_w2_wcar.pdf}}
\caption{Average WCAR with Facebook traffic traces using (a) small and (b) large-scale networks. The values of $(p_2,w_2)$ are set to $(0.2,2)$. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Fb:WCAR}}
\end{figure}



Figs.~\ref{fig:Off:Fb:ClassCAR:Small} and \ref{fig:Off:Fb:ClassCAR:Big} shows the average CAR of each coflow class with Facebook traffic traces using small and large-scale networks, with $(p_2,w_2) = (0.5,2)$.  We can  see that   \wdcoflow\ and \wdcoflowDP\  achieve big improvement for Class 2, while \csdp\ obtains worse  performance for both classes. The reason
for this is that  \csdp\  schedules coflows only according to
the network conditions, while  \wdcoflow\ and \wdcoflowDP\  consider both network
conditions and importance of coflows.  Under   \wdcoflow\ and \wdcoflowDP\,
coflows with higher weight have higher priority, thus the average WCAR will greatly increase.


\begin{figure}[h]
\centering
\subfloat[{Small-scale networks.\label{fig:Off:Fb:ClassCAR:Small} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_fb_m10_p5_w2_classcar.pdf}}
\subfloat[{Large-scale networks.\label{fig:Off:Fb:ClassCAR:Big} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_offline/off_fb_m100_p5_w2_classcar.pdf}}
\caption{Average per-class CAR with Facebook traffic traces using (a) small-scale and (b) large-scale networks. Each point in the x-axis represents the network $[M,N]$. \label{fig:Off:Fb:ClassCAR}}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Online Setting  \label{sec:Eva:On}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We now present numerical results comparing
the performance of the online version of \wdcoflow\ and \wdcoflowDP\  against the online version of \csdp. The results are obtained on instances generated using our workload generator, with $50$ machines and $3000$ coflow arrivals. 
Coflow arrivals follow a Poisson process with an average rate of $\lambda$ (coflows/time slot). The arrival rate $\lambda$ varies from $2$ to $10$, and the probability and weight of Class-2 coflows are fixed to respectively $0.5$ and $10$. For the sake of comparison, we have used the greedy allocation algorithm (see the beginning of Sec.~\ref{sec:Evaluation}) to perform the resource allocation after obtaining the $\sigma$-order. The average performance of all algorithms are calculated over $40$ runs with $40$ different instances of the same setting.

 %from the comparing algorithms and calculate the CCTs and the corresponding WCAR of all coflows

Fig.~\ref{fig:On:Syn:ChangeLambda:WCAR} and \ref{fig:On:Syn:ChangeLambda:ClassCAR} illustrate the WCAR and per-class CAR of coflows. We observe that  \wdcoflow\ and \wdcoflowDP\ improve  the average WCAR as compared to \csdp. For instance, with $\lambda = 4$, the WCAR improvement of \wdcoflow\ and \wdcoflowDP\ compared to \csdp\ are respectively $7\%$ and $12\%$. 
In addition, they greatly improve the CAR for Class $2$  for all $\lambda$ compared to \csdp\ (see Fig.~\ref{fig:On:Syn:ChangeLambda:ClassCAR}). This shows that our proposed heuristics consider both network conditions and the importance of coflows to determine the $\sigma$-order that allows to greatly improve the CAR of Class $2$.    


\begin{figure}[h]
\centering
\subfloat[{Average WCAR.\label{fig:On:Syn:ChangeLambda:WCAR} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_online/on_syn_m50_c3000_p8_w10_changeLambda.pdf}}
\subfloat[{Per-class CAR.\label{fig:On:Syn:ChangeLambda:ClassCAR} }]{
\includegraphics[width=4.4cm, height=3.6cm]{figuresw/results_online/on_syn_m50_c3000_p5_w2_classcar.pdf}}
\caption{(a) Average WCAR and (b) per-class CAR with synthetic traffic traces when varying $\lambda$ and fixing $p_2=0.5$ and $w_2=2$. \label{fig:On:Syn:ChangeLambda}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/ProbStat.tex <==
%!TEX root=TDPCS.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Problem Statement 
\section{Problem Statement and Theoretical Analysis 
\label{sec:Problem-Statement}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we present the system model and formulate the acceptance rate maximization problem for a given input set of coflows. Table~\ref{tab:Prob:Notations} summarizes the main notations used throughout the paper.
%The datacenter network can be modeled as a directed graph, $\cG = (\cV, \cL)$, where $\cL$ is the port set and $\cV$ is the node set. 
The datacenter network (or datacenter fabric) is represented as a \textit{Big-Switch} model \cite{Chowdhury2014}, a non-blocking switch whose ingress (egress) port $\ell$ has capacity $B_{\ell}$ equal to the corresponding bandwidth inbound (outbound) capacity to connect servers to the top-of-rack (ToR) switch. Actually, due to large bisection capacity and customary usage of load balancing routing algorithms such as, e.g., ECMP, traffic congestion is typically observed only at the rack access ports leading to the ToR switches.

We consider a batch of $N$ coflows $\cC = \{1, 2, ..., N\}$. A coflow is a collection of flows, in which each flow represents a shuffle connection over a pair of fabric ingress-egress ports. Denote $\cF_{k}$ as the set of flows of coflow $k \in\cC$ and assume that the volume $v_{k,j}$ of each flow $j \in \cF_k$ is known. For the sake of clarity, we suppose that all coflows arrive at the same time, i.e., their release time is zero. Also, each coflow $k$ is subject to a completion deadline $T_k$. Similarly, we let $\cF_{\ell,k}$ be the set of flows in $\cF_{k}$ which uses port $\ell \in \cL$ either as ingress port or as egress port. The total volume of data sent by coflow $k$ on port $\ell$  is then given by  $\hv_{\ell,k}=\sum_{j \in \cF_{\ell,k}} v_{k,j}$. Let $p_{\ell,k}$ be the transfer completion time in isolation, i.e., at full rate, of coflow $k$ at port $\ell$, which is given by $p_{\ell,k} = \hv_{\ell,k} / B_\ell$. %\frac{\hv_{\ell,k}}{B_\ell}.
%In datacenters, coflows can be divided into two categories; deadline coflows and non-deadline coflows. The importance of meeting coflow deadline has been illustrated in the literature \cite{} and their arguments are often generated by  Sensitive Applications that have strict latency requirements.  Hence the goal of the paper is: how to schedule coflows to maximizes the coflow deadline satisfaction, i.e., the number of coflows that can  meet their deadline. 
Let $r_{k,j}(t) \in \mathbb {R}_{+}$ be the rate allocated to flow $j\in {\cal F}_k$ at time $t$. The CCT of coflow $k$, denoted as $c_k$, thus writes
\begin{equation}
c_k = \max_{j\in {\cal F}_k}  \frac{v_{k,j}}{\bar r_{k,j}}, \mbox{ where}~  \bar{r}_{k,j} =\frac{1}{CT_{k,j}} \int_0^{CT_{k,j}} r_{k,j} (t) \diff{t},
\end{equation}
% where 
% $$
% \bar{r}_{k,j} =\frac{1}{CT_{k,j}} \int_0^{CT_{k,j}} r_{k,j} (t) \diff{t},
% $$
and $\bar r_{k,j}$ is the average rate of flow $j$ through its lifetime and  $CT_{k,j}$ is its completion time. This quantity rules the dispatching time for the volume traversing the so-called coflow bottleneck which determines the CCT of the said coflow. Hence coflow $k$ satisfies a prescribed deadline $T_k$ when $c_k\leq T_k$, i.e., its last flow completes before.

Let $z_{k} \in \{0,1\}$ be a variable indicating whether coflow $k$ finishes before $T_k$ or not. Maximizing the number of coflows meeting their deadline corresponds to maximizing the sum of the variables $\{z_k\}$ subject to the constraint of bandwidth capacity at ingress and egress ports. The CAR maximization problem can be formulated as 
\begin{align}
\underset{r}{\mathrm{max}}\enskip & \sum_{k\in\mathcal{C}}  z_{k} \tag{CAR}\label{prob:CAR}\\
\mathrm{s.t.}\enskip 
% & r_{k,j}(t) \geq 0,\label{prob:CAR-1}\\
& \sum_{k \in \mathcal{C}} \sum_{j\in\mathcal{F}_{k,l}} r_{k,j}(t)\leq  B_{\ell}, \quad \forall \ell \in \mathcal{L}, \forall t \in \mathcal{T}, \label{prob:CAR-1} \\
& \int_0^{T_k} r_{k,j} (t) \diff{t} \geq  v_{k,j} z_k, \quad \forall j \in \mathcal{F}_k, \forall k \in \mathcal{C}, \label{prob:CAR-2}
%& \sum_{t \in [0, T_k]}  r_{k,j}(t) \geq  v_{k,j} z_k, \quad \forall j \in \mathcal{F}_k, \forall k \in \mathcal{C}, \label{prob:CAR-2}
\end{align}
%where $x^{k,j}_{\ell} \in \{0,1\}$ is an indicator of whether flow $j$ passes through port $\ell$.
Constraint \eqref{prob:CAR-1} expresses that, within the time horizon $\cT$, the total rate that port $\ell$ assigns to flows at any instant $t$ cannot exceed its capacity $B_{\ell}$. Constraint \eqref{prob:CAR-2} ensures that the data of flows of each \textit{accepted} coflow $k$ should be completely transmitted before the deadline $T_k$. 
\begin{lemma}[Proposition 1 in \cite{Tseng2019}]
\label{lem:problem-complexity}
There exists a polynomial time reduction of \ref{prob:CAR} to the problem of minimizing the number of late jobs in a concurrent open shop \cite{Lin2007}. Hence, the CO-CAR problem is \textit{NP}-hard. 
\end{lemma}


\begin{center}
\begin{table}[t]
\caption{Main notations. \label{tab:Prob:Notations}}
\footnotesize
\centering{}%
\begin{tabular}{cl}
\toprule 
{Symbol} & {Description} \tabularnewline
\cmidrule[0.4pt](lr{0.12em}){1-1}%
\cmidrule[0.4pt](lr{0.12em}){2-2}%
$\cL$ & set of fabric ports\tabularnewline
% $\cI$ & set of ingress ports\tabularnewline
% $\cO$ & set of egress ports\tabularnewline
$M$ & number of machines, $M = |\cL|/2$\tabularnewline
$B_{\ell}$ & available bandwidth of port $\ell\in\mathcal{L}$\tabularnewline
% $r_{\ell}$ & release time of port $\ell\in\mathcal{L}$\tabularnewline
$\cC$ & set of coflows. $\cC$ has cardinality of $N$\tabularnewline
$\sigma$ & scheduling order of coflows, $\sigma=\left\{ \sigma_{1},\cdots,\sigma_{N-1},\sigma_{N}\right\} $\tabularnewline
$T_{k}$ & deadline of coflow $k$\tabularnewline
$\cF_k$ ($\cF_{\ell,k}$) & set of flows of coflow $k$ (that use port $\ell$) \tabularnewline
$v_{k,j}$ & volume of flow $j \in \cF_k$ of coflow $k$\tabularnewline
$\hv_{\ell,k}$ & total volume transmitted by coflow $k$ on port $\ell$\tabularnewline
$p_{\ell,k}$ & processing time of coflow $k$ on port $\ell$\tabularnewline
$c_{k}$ ($c_{\ell,k}$) &  completion time of coflow $k$ on port $\ell$ \tabularnewline
${CT}_{k,j}$ & completion time of flow $j$ of coflow $k$ \tabularnewline
\bottomrule
\end{tabular}
\end{table}
\end{center}
The problem \ref{prob:CAR} is generalized to the weighted case in Sec.~\ref{sec:weighted}, to assign different priority to the admission of different coflows. Now, we discuss the structure of the \ref{prob:CAR} problem and how to overcome the limitations of state of art solutions using a specific example. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motivating Example}
\label{subsec:Motivating-Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
% \begin{figure}[H]
% \centering
% \vspace*{-0cm}
% \hspace*{-0cm}
% \includegraphics[clip,width=9cm,height=4.5cm]{Fabric_Example_Dcoflow.pdf}
% %\vspace{-0cm}
% \caption{Motivating example with a Big Switch fabric composed of 4 ingress/egress ports connecting to $4$ machines.  Flows in ingress ports are organized by destinations and color-coded by coflows. The example has 5 coflows. Coflow $C1$ (blue) has $4$ flows, with each ingress port sending $1+\varepsilon$ units of data to one egress port and its deadline is $1+\varepsilon$;
% coflows $C2$ (green), $C3$ (red), $C4$ (orange)  and $C5$ (purple) have a single flow each sending $1$ units of data and their deadline is 2 }
% \label{fabric1}
% \end{figure}


We will take $\mathtt{CS\text{-}MHA}$~\cite{Luo2016} as our starting point to address the WCAR problem. $\mathtt{CS\text{-}MHA}$  has introduced a new direction to solve the scheduling problem by means of a static coflow prioritisation. The prioritisation is used in order to approximate the solution of the coflow scheduling problem that maximizes the CAR. $\mathtt{CS\text{-}MHA}$ computes the scheduling orders at each port using the Moore-Hodgon's algorithm which also determines the set of admitted coflows at each port $\ell\in{\mathcal{L}}$.  Since different ports could have different  sets of admitted coflows, a coflow is admitted if it is admitted at all ports. For all rejected coflows, a second round is applied to check if some rejected coflows can actually satisfy their deadline. The algorithm selects a coflow with the minimum bandwidth required at the bottleneck port since it is more likely to catch up with its deadline. 

The simple example depicted in Fig.~\ref{fig:Example} illustrates the limitations of  $\mathtt{CS\text{-}MHA}$. It uses the standard \emph{Big-Switch} model to abstract a datacenter fabric: the example will be used as a running example throughout the paper. The instance contains $5$ coflows: $C_{1}$ has $4$ flows and $C_{2}$, $C_{3}$, $C_{4}$ and $C_{5}$ each have one flow. To ease the presentation, the flows are organzed in virtual output queues at the ingress ports. The virtual queue index represents the flow output port, modulo the number of machines. The numbers on the flows' representations correspond to their \textit{normalized} volumes. All fabric ports have the same \textit{normalized} bandwidth of $1$. At the first iteration, $\mathtt{CS\text{-}MHA}$ computes the scheduling order  on each port using Moore-Hodgson algorithm \cite{Moore1968}, which is based on the \textit{Earliest Due Date} rule and is known to minimize the number of missed deadlines on a single machine (or \textit{port} in the coflow context). Since coflow $C_{1}$ uses all ports and has the smallest deadline ($T_{1} = 1$), then at each port, $C_{1}$ will be scheduled first. As consequence, all other coflows are rejected since they cannot satisfy their deadline when scheduled after $C_{1}$. Given that coflow scheduling, the CAR is $\frac{1}{5}$. However, an optimal scheduling solution would be $\{C_{2}, C_{3}, C_{4}, C_{5}, C_{1}\}$ or any combination that has coflow $C_{1}$ as the last one to be scheduled. The latter scheduler attains a CAR of $\frac{4}{5}$. From this example, we can see that $\mathtt{CS\text{-}MHA}$ can be made arbitrarily worse compared to the optimal solution. 

The above example can easily be extended to show that in the worst-case scenario, the CAR of  $\mathtt{CS\text{-}MHA}$ can be made arbitrarily small (as close to $0$ as needed). Consider $M$ machines, coflow $C_1$ that uses all ports, and coflows $C_2,\hdots, C_M$ with one flow each. The other parameters hold unchanged. 

Finally, the key observation is that $\mathtt{CS\text{-}MHA}$ neglects the impact that a coflow may have on the other coflows on several ports. Indeed, a coflow causing multiple deadlines to be missed should have lesser priority, even when its deadline is the earliest. When this fact is neglected, the coflow ordering is misjudged and the final schedule can severely degrade the CAR with respect to an optimal solution. Starting from this observation and propose a new $\sigma$-order scheduler, called $\mathtt{DCoflow}$ which solves the \ref{prob:CAR} problem in the unweighted case and it is generalized to the \ref{prob:ILP} problem later on. 

In particular, with respect to the example, it can be seen that the CAR obtained using $\mathtt{CS\text{-}MHA}$  and $\mathtt{DCoflow}$ are $\frac{1}{M}$, $\frac{M-1}{M}$, respectively.  In this setting, the CAR obtained using $\mathtt{CS\text{-}MHA}$  is close to zero when $M$ is high. while  using  $\mathtt{DCoflow}$, the CAR is close to one.

\begin{figure}[t]
\centering
\includegraphics[width=0.65\columnwidth]{fig_coflow/intro/fig_motivation_example.pdf}
\caption{Motivating example with a Big-Switch fabric composed of $4$ ingress/egress ports connecting to $4$ machines. Flows in ingress ports are organized by destinations and are color-coded by coflows. The example has $5$ coflows. Coflow $C_1$ (blue) has $4$ flows, with each ingress port sending $1$ units of data to one egress port: its deadline is $1$;
coflows $C_2$ (green), $C_3$ (red), $C_4$ (orange) and $C_5$ (purple) have a single flow, each sending $(1+\varepsilon)$ unit of data. The deadline of these coflows is $2$.  \label{fig:Example}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Coflow Ordering 
\label{subsec:Coflow-Ordering}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The problem \ref{prob:CAR}  implicitly depends on the CCT. An alternative approach to maximize the CAR is to {\em order} the coflows in some appropriate way, and then to leverage the priority forwarding mechanisms of the underlying transport network \cite{Agarwal2018}.

%A common drawback of most existing works on coflow scheduling is that they assume that the transport layer is able to enforce the per-flow rate allocation computed by the scheduling algorithm. In practice, however, this is seldom the case as the rates are computed using an overly simplified model of the transport network. As proposed in \cite{Agarwal2018} for the minimization of the average coflow completion time (CCT), an alternative approach is to order the coflows in some appropriate order, and then to leverage the priority forwarding mechanisms of the underlying transport network.

In this approach, %the goal is to determine an ordering $\sigma: \{1, 2, \ldots, N\} \rightarrow \cC$ of coflows, which prescribes that coflow $\sigma_{k}$ should be transmitted before coflow $\sigma_{k+1}$, for all $k \in [1, N-1]$. 
once such an ordering $\sigma$ is determined, it is enough to adopt work-conserving transmission policies and use forwarding priorities in such a way that a flow $j \in \cF_{\sigma_{k}}$ is blocked if and only if either its ingress or egress port is busy serving a flow $j' \in  \cF_{\sigma_{k'}}$ for some $k' < k$, i.e., a flow of a coflow with higher priority according to $\sigma$. Such a flow scheduling is called \emph{$\sigma$-order-preserving}. 

The formulation of problem \eqref{prob:CAR} can be transformed into an Integer Linear Program (ILP) as follows. %We define the binary variable $\delta_{i,k}$ as $1$ if coflow $i$ is scheduled before coflow $k \neq i$, and $0$ otherwise. The ordering of coflows can then be modeled using the following standard disjunctive constraints.
We define the binary variable $\delta_{i,k}$ as $1$ if coflow $i$ has higher priority than coflow $k \neq i$, and $0$ otherwise. The ordering of coflows can then be modeled using the following standard disjunctive constraints
\begin{eqnarray}
\delta_{k,k'} + \delta_{k',k} & = & 1, \quad \forall k,k' \in \cC, \label{eq:order-disjunct-1} \\
\delta_{k,k'} + \delta_{k',k"} + \delta_{k",k} & \leq & 2, \quad \forall k,k',k" \in \cC. \label{eq:order-disjunct-2}
\end{eqnarray}

It should be clear that the ordering $\sigma$ can easily be derived from the variables $\{ \delta_{k,k'} \}_{k,k' \in \cC}$. This ordering should be such that as many coflows as possible are accepted, that is, $\sum_{i \in \cC} z_k$ is maximized. A central difficulty here is to compute the completion time of a coflow, which stems from the fact that data transmissions on the various ports are not independent: the transmission of a flow may be blocked until the ingress port becomes available even if the egress port is idle, and vice versa. However, assuming that the ports are independent, we can obtain a lower bound on the completion time of coflow $k$ on port $\ell$ as follows
\begin{equation} \label{eq:lower-bound-CCT}
c_{\ell,k} \geq \sum_{k' \neq k} p_{\ell,k'} \delta_{k',k} z_{k'} + p_{\ell,k}, \quad \forall \ell \in \cL, k \in \cC.
\end{equation}
This lower bound assumes that the transmission of coflow $k$ on port $\ell$ can start as soon as all flows of all coflows $k'$ scheduled before $k$ have been transmitted on port $\ell$. Note that the above constraint is not linear due to the product $\delta_{k',k} z_{k'}$. However, it can easily be linearized by introducing binary variables $y_{k',k}$ satisfying the constraints 
\begin{equation}
y_{k',k} \leq z_{k'}; 
\quad y_{k',k} \leq \delta_{k',k}; 
\quad y_{k',k} \geq z_{k'}+\delta_{k',k} - 1, \label{eq:y1} 
% y_{k',k} & \leq \delta_{k',k}, \label{eq:y2} \\
% y_{k',k} & \geq z_{k'}+\delta_{k',k} - 1, \label{eq:y3}
\end{equation}
\eqref{eq:lower-bound-CCT} thus becomes
\begin{equation} \label{eq:lower-bound-CCT-new}
c_{\ell,k} \geq \sum_{k' \neq k} p_{\ell,k'} y_{k',k} + p_{\ell,k}, \quad \forall \ell \in \cL, k \in \cC.  
\end{equation}
A lower bound on the completion time of coflow $k$ is then obtained as $c_k = \max_{\ell \in \cL} c_{\ell,k}$, and this coflow can meet its deadline only if $c_k \leq T_k$. The deadline constraint can then be described as
\begin{equation} \label{eq:deadline-constraint}
c_{\ell,k} \leq T_k z_k, \quad \forall \ell \in \cL, k \in \cC.  
\end{equation}
We can thus obtain an upper bound on the number of accepted coflows by solving the following ILP, 
\begin{equation} \label{prob:CAR-ILP}
\mathrm{max}\enskip \sum_{k\in\mathcal{C}} z_{k}\tag{CAR-ILP}, \quad
\mathrm{s.t.}\enskip (\ref{eq:order-disjunct-1}, \ref{eq:order-disjunct-2}, \ref{eq:y1}, \ref{eq:lower-bound-CCT-new}, \ref{eq:deadline-constraint}).\nonumber
\end{equation}
% \begin{align}
% \mathrm{max}\enskip & \sum_{k\in\mathcal{C}}z_{k}\tag{P2}\label{prob:ILP}\\
% \mathrm{s.t.}\enskip & \delta_{k,k'}+\delta_{k',k}=1,\quad\forall i,k\in\mathcal{C},\label{prob:ILP-1}\\
%  & \delta_{k,k'}+\delta_{k',k"}+\delta_{k",k}\leq2,\quad\forall k,k',k"\in\mathcal{C},\label{prob:ILP-2}\\
%  & y_{k',k}\leq z_{k'},\quad\forall k,k'\in\mathcal{C},\label{prob:ILP-3}\\
%  & y_{k',k}\leq\delta_{k',k},\quad\forall k,k'\in\mathcal{C},\label{prob:ILP-4}\\
%  & y_{k',k}+1\geq z_{k'}+\delta_{k',k},\quad\forall k,k'\in\mathcal{C},\label{prob:ILP-5}\\
%  & c_{k}\geq\sum_{k'\neq i}p_{\ell,k'}y_{k',k}+p_{\ell,k},\quad\forall\ell\in\mathcal{L},k\in\mathcal{C},\label{prob:ILP-6}\\
%  & z_{k}c_{k}\leq T_{k},\quad\forall k\in\mathcal{C},\label{prob:ILP-7}\\
%  & \delta_{k',k},y_{k',k}\in\left\{ 0,1\right\} ,\quad\forall k,k'\in\mathcal{C},\label{prob:ILP-8}\\
% %
%  & z_{k}\in\left\{ 0,1\right\} ,\quad\forall k\in\mathcal{C}.\label{prob:ILP-9}
% \end{align}
It is easy to verify that Problem~\ref{prob:CAR-ILP} is still \textit{NP}-hard and so that it may become unfeasible to find an optimal solution in large-scale datacenter networks. In the next section, we hence propose an efficient heuristic algorithm to determine %the order in which coflows must finish in order to maximize the coflow acceptance rate. 
the priority order among coflows in order to maximize the coflow acceptance rate. 


==> sections/Weighted.tex <==
% !TEX root =  ./TDPCS.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{DCoflow for weighted coflows}\label{sec:weighted}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Up to now, it was assumed that the goal was to maximize the number of accepted coflows satisfying their deadline constraints. In this section, we shall assume that a weight $w_k$ is assigned to each coflow $k \in \mathcal{C}$ and that the goal is to maximize the total weight of coflows that finish before their deadlines. In other words, we shall consider the following optimization problem:

\begin{equation} \label{prob:ILP}
\mathrm{max}\enskip \sum_{k\in\mathcal{C}} w_k z_{k}\tag{WCAR}, \quad
\mathrm{s.t.}\enskip (\ref{eq:order-disjunct-1}, \ref{eq:order-disjunct-2}, \ref{eq:y1}, \ref{eq:lower-bound-CCT-new}, \ref{eq:deadline-constraint}).\nonumber
\end{equation}

In a natural economic interpretation of the above problem, one can view the weight $w_k$  as the price a user is willing to pay to the cloud provider if its coflow $k$ completes before its deadline. In the WCAR problem, the cloud provider then maximizes its revenue given the prices (weights). 

It immediately follows from Lemma \ref{lem:problem-complexity} that the the WCAR problem is \textit{NP}-hard. We show below how to extend the \dcoflow \ algorithm given in Algorithm \ref{algo:DCoflow} to  maximize the total weight of accepted coflows.  We first present a simple dynamic programming algorithm for minimizing the weighted number of late jobs on a single machine in Section \ref{subsec:dp-algorithm}. This algorithm is a key ingredient of our new heuristic, named  \wdcoflowDP,  to minimize the weighted number of late coflows.

% Minimization of the weighted number of late jobs
\subsection{Minimization of the weighted number of late jobs on a single machine}
\label{subsec:dp-algorithm}
Consider a set of $n$ jobs that has to be non-preemptively processed on a single machine. All jobs are available at time $0$ and job $j=1,\ldots,n$ is characterized by its processing time $p_j$, its deadline $T_j$ and its integer weight $w_j$. The goal is to minimize the weighted number of late jobs, a problem usually referred to as $1 \Vert \sum w_j U_j$. This problem can be formulated as the following integer linear programming problem:

\begin{align}
    \mbox{maximize} & \sum_{j=1}^n w_j z_j \label{eq:late-jobs-obj} \\
    \mbox{subject to:} & \nonumber \\
    & \sum_{j=1}^k p_j z_j \leq T_k, \quad k=1,\ldots,n \label{eq:late-jobs-cstr1} \\
   & z_j \in \{0,1\}, \quad j=1,\ldots,n \label{eq:late-jobs-cstr2}
\end{align}

More precisely, problem \eqref{eq:late-jobs-obj}-\eqref{eq:late-jobs-cstr2} finds a maximum-weight feasible set of jobs, which is clearly equivalent to minimizing the weighted number of late jobs. Note that when all deadlines are equal, all inequalities \eqref{eq:late-jobs-cstr1} are implied by the last one, $\sum_{j=1}^n p_j z_j \leq T_n$, and the problem reduces to the ordinary knapsack problem. Since the latter problem is known to be NP-hard, it follows that the problem $1 \Vert \sum w_j U_j$ is also NP-hard. Nevertheless, this problem can be solved by a dynamic programming algorithm within a pseudo-polynomial time bound of $O(nW)$, where $W=\sum_j w_j$, as we now explain.

%Minimizing the weighted number of late jobs is clearly equivalent to finding a maximum-weight feasible set of jobs. As it includes the ordinary knapsack problem as a special case, this problem is NP-hard. Nevertheless, it can be solved by a dynamic programming algorithm within a pseudo-polynomial time bound of $\cO(nW)$, where $W=\sum_j w_j$, as we now explain.

Without loss of generality, we assume that jobs are numbered in the EDD order, that is, $T_1 \leq T_2 \leq \ldots, T_n$. Let $P^{(j)}(w)$ denote the minimum total processing time for any feasible subset of jobs $1,\ldots,j$ that has total weight $w$. Initially, $P^{(0)}(0)=0$ and $P^{(0)}(w)=+\infty$ for all $w \in \{1,2,\ldots,W\}$. In the subsequent $n$ iterations $j=1,2,\ldots,n$, the variables $P^{(j)}(w)$ are computed as 

\begin{equation}
P^{(j)}(w) =   \min \left \{ P^{(j-1)}(w), \ P^{(j-1)}(w-w_j)+p_j \right \},
\label{eq:dp-iter-eq1}
\end{equation}

\noindent if $P^{(j-1)}(w-w_j)+p_j\leq T_j$, and as 

\begin{equation}
P^{(j)}(w) =  P^{(j-1)}(w),
\label{eq:dp-iter-eq2}
\end{equation}

\noindent otherwise. At the end of the algorithm, the maximum weight of a feasible set is the largest value of $w$ such that $P^{(n)}(w)$ is finite. The maximum-weight feasible set is easily obtained with standard backtracking techniques. Finally, we note that, provided that the processing times and job weights are oppositely ordered, the problem $1 \Vert \sum w_j U_j$ can be solved in $O(n \log n)$ time with the Moore-Hogdson algorithm~\cite{Moore1968}.

%\begin{equation}
%P^{(j)}(w) = \begin{cases}
%    \min \left \{ P^{(j-1)}(w), \ P^{(j-1)}(w-w_j)+p_j \right \} & \mbox{if } P^{(j-1)}(w-w_j)+p_j\leq T_j,\\
%    P^{(j-1)}(w) & \mbox{otherwise,}
%    \end{cases} 
%\label{eq:dp-iter}
%\end{equation}

% Fast Scheduling of Weighted Coflows with Deadlines

\subsection{Coflow Rejection Rule \label{subsec:coflow-rejection-rule}}
The coflow rejection rule is used to determine which coflow will be rejected and it is based on a slightly  modified  schedulability condition  used by $\mathtt{DCoflow}$ in Sec.~\ref{sec:heuristic}.  

 Given a set $\cS$ of coflows and subset of $\cR$ of  $ \cS$, and assuming that $p_{\ell,k}=0$ if coflow $k$ does not use port $\ell$, define for each port $\ell \in \cL$ the quantity $I_\ell \left ( \cS \right ) = \sum_{k \in \cS}p_{\ell,k} T_k - f_\ell \left (\cS \right )$. 
 % where  $f_\ell \left ( \cS \right ) = \frac{1}{2} \left \{ \left ( \sum_{k \in {\mathcal S}} p_{\ell,k} \right )^2 + \sum_{k \in {\mathcal S}} p_{\ell,k}^2 \right \}$. 
 The set $\cL^\star=\left \{ \ell \in \cL \ : I_\ell(\cS) < 0 \right \}$ then represents the set of ports on which at least one coflow is late, whatever the order in which the coflows are (locally) processed. Hence, if $\cL^\star \neq \varnothing$, at least one coflow $k^\star$ using one or more ports in $\cL^\star$ should be removed from $\cS$ for the remaining coflows to meet their deadlines.  
 
 
If there is only one port $\ell$ in $\cL^\star$, a natural choice is to choose $k^\star$ so as to maximize the quantity $I_\ell \left ( \cS \setminus \{ k^\star \} \right )$ in the hope that it becomes positive. It is easy to show from the definition of $I_\ell \left ( \cS \right )$ that 
$
I_\ell \left ( \cS \setminus \{ k' \} \right )=I_\ell \left ( \cS \right ) + \Psi_{\ell,k'},
$
where $\Psi_{\ell,k'}=p_{\ell,k'} \left ( \sum_{k \in \cS} p_{\ell,k} - T_{k'} \right )$.    
As coflows with small weights should be rejected in priority, we choose $k^\star \in \mbox{argmax}_{k\in \cR} \frac{1}{w_k} \Psi_{\ell,k}$. In words, this rule dictates to reject a coflow $k^\star\in \cR$ with a small weight $w_{k^\star}$ and which has either a large processing time $p_{\ell,k^\star}$ or a large deadline violation $\sum_{k \in \cS} p_{\ell,k} - T_{k^\star}$, or both.

When there is more than one port in $\cL^\star$, a straightforward extension of  the previous rule is to choose a coflow $k^\star$ with a small weight so as to maximize $\sum_{\ell \in \cL^\star} I_\ell \left ( \cS \setminus \{ k^\star \} \right )$. In this case, we choose the coflow $k^\star$ in $\cR$ with the largest value of the index  $\frac{1}{w_k^\star} \sum_{\ell \in \cL^\star} \Psi_{\ell,k^\star}$. An obvious advantage of this simple rule is that it allows to account for the impact of the removal of coflow $k^\star$ on all ports $\ell \in \cL^\star$ used by this coflow.   

We note that the role of the subset  $\cR$ is specified in the next section to designate the candidate coflows among which we will choose a coflow to schedule.  Let us recall in the $\mathtt{DCoflow}$ algorithm, the candidates at each step,  are those who use the bottleneck. 

\subsection{Fast Scheduling of Weighted Coflows with Deadlines \label{subsec:dcoflow-offline}}
The proposed offline algorithm, which is called \wdcoflowDP,   takes as input a set $\cC=\{1,2,\ldots,N\}$ of coflows, which are all available at time $0$, and computes as output the scheduling order of accepted coflows. Due to the lack of space, we do not give the pseudo-code of the algorithm, which is a direct adaptation of Algorithm \ref{algo:DCoflow}. We only indicate the main steps of  \wdcoflowDP, highlighting the main differences with Algorithm \ref{algo:DCoflow}.

As for \dcoflow, there are two main phases in \wdcoflowDP. In the first phase, the algorithm works in rounds and at each round it either accepts one coflow or rejects one. The selected coflow is then removed from the current set of coflows $\cS$, which is initialized to $\cC$. \wdcoflowDP \  uses two vectors $\sigma$ and $\sigma^\star$ to keep track of the accepted/rejected coflows at each iteration: $\sigma_{N-n+1}$ is the identity of the coflow selected at iteration $n=1,2,\ldots,N$, and $\sigma^{\star}_{N-n+1}$ is the identity of the coflow rejected at that iteration, if any (otherwise, by convention, we set $\sigma^{\star}_{N-n+1} = 0$).

At each round $n$, \wdcoflowDP \  sweeps through the set of coflows $\cS$ to compute the total completion time $t(\ell)=\sum_{k \in \cS} p_{\ell, k}$ of each port $\ell$. It then determines the bottleneck port $\ell_b$, that is, the port $\ell$ with the largest completion time $t(\ell)$. Let $k'$ be the coflow using port $\ell_b$ with the largest deadline. If $t(\ell_b) \leq T_{k'}$, then coflow $k'$ can be scheduled as the last one on port $\ell_b$ and still satisfies its deadline. This coflow is therefore accepted by the algorithm and we set $\sigma_{N-n+1} = k'$ and $\sigma^{\star}_{N-n+1} = 0$. If on the contrary $t(\ell_b) > T_{k'}$, this implies that at least one coflow among those using the bottleneck port will be late and therefore one of these coflows has to be rejected. \wdcoflowDP \  then uses the DP algorithm discussed in Section \ref{subsec:dp-algorithm} for minimizing the weighted number of late coflows on port $\ell_b$. Let $\cR$ be the set of coflows rejected by the DP algorithm. \wdcoflowDP \ then chooses the coflow $k^\star \in \cR$ to be rejected using the rejection rule described in Sec.~\ref{subsec:coflow-rejection-rule}, and sets $\sigma_{N-n+1} = \sigma^{\star}_{N-n+1} = k^\star$.

The second phase of \wdcoflowDP \ is a post-processing phase intended at accepting unduly rejected coflows. Indeed, some coflows in $\sigma^{\star}$ could have been accepted if certain coflows that were rejected later would have been rejected earlier. To handle such cases, we use the function $\mathtt{RemoveLateCoflows}$ proposed in \cite{Dcoflow22}. Briefly, in this second phase, \wdcoflowDP \ sweeps through the vector $\sigma^{\star}$, skipping the values $n$ such that $\sigma^{\star}_{n} = 0$, and for each pre-rejected coflow $k^\star=\sigma^{\star}_{n}$, it estimates its CCT considering only the coflows scheduled before $k^\star$ in the order $\sigma$. If $k^{\star}$ cannot meet its deadline, it is permanently removed from $\sigma^{\star}$ and $\sigma$. Otherwise, coflow $k^\star$ is definitely accepted in the order $\sigma$. At the end of  the second phase of \wdcoflowDP, the estimated CCT of all coflows appearing in the order $\sigma$ is at most their deadline.

There are two main differences between \wdcoflowDP \ and \dcoflow.  The first one is the incorporation of coflow weights in the coflow rejection rule. A similar rule was used in \cite{Dcoflow22}, but assuming that all coflow weights are equal. The second difference is the use of the DP algorithm which plays the role of a filter that  restricts the choice of coflows that can be rejected. We note that  the main advantage of using the DP algorithm is that, as is easily proven,  \wdcoflowDP \  produces an optimal schedule minimizing the weighted number of late coflows when there is only one input port and one output port. This was not the case of Algorithm 1 in \cite{Dcoflow22}, even for coflows with equal weights. However, the downside is that the running time of  \wdcoflowDP \  is only pseudo-polynomial in the sum of coflow weights. Therefore, in the following, we shall also consider a version of the algorithm in which the DP filter is not enabled. We shall refer to this version as simply \wdcoflow \ and compare its performance to that of  \wdcoflowDP. It is easy to see that the complexity of \wdcoflow \ is  $\cO(N^2)$.


